Deconstructing the Blockchain to Approach Physical Limits

Transaction throughput, confirmation latency and confirmation reliability are fundamental performance measures of any blockchain system in addition to its security. In a decentralized setting, these measures are limited by two underlying physical network attributes: communication capacity and speed-of-light propagation delay. Existing systems operate far away from these physical limits. In this work we introduce Prism, a new proof-of-work blockchain protocol, which can achieve 1) security against up to 50% adversarial hashing power; 2) optimal throughput up to the capacity C of the network; 3) confirmation latency for honest transactions proportional to the propagation delay D, with confirmation error probability exponentially small in CD ; 4) eventual total ordering of all transactions. Our approach to the design of this protocol is based on deconstructing the blockchain into its basic functionalities and systematically scaling up these functionalities to approach their physical limits.

==> Approach.tex <==
\section{Approach}
\label{sec:approach}

A critical parameter of any PoW blockchain protocol is the mining rate, i.e. the rate at which puzzles are successfully solved (also called the PoW solution rate). The mining rate can be easily controlled via adjusting the difficulty of the puzzle, i.e. the threshold at which the hash inequality needs to be satisfied. The mining rate has a profound impact on both the transaction throughput and confirmation latency. Large mining rate can potentially increase the transaction throughput by allowing transactions to be processed quicker, and can potentially reduce the confirmation latency by increasing the rate at which votes are cast to confirm a particular transaction. However, increasing the mining rate has the effect of increasing the amount of forking in the blocktree,  because blocks mined by different nodes within the network delay cannot be mined on top of each other and are hence forked. This de-synchronization slows down the growth rate of the longest chain, making the system more vulnerable to private chain attacks, and decreasing the security of the  protocol. Indeed, one reason why \bitcoin is (comparatively) secure is that the mining rate is set to be very small, one block per $10$ minutes. At the current \bitcoin block size of $1$ Mbytes, this corresponds to a generated traffic of about $13$ kbits/second, much less than the capacity of typical communication links \cite{statoshi}. Thus, \bitcoinnosp's performance is security-limited, not communication-limited, and far away from the physical limits.


\begin{figure}
  \centering
  \includegraphics[width=.8\linewidth]{figures/Messy_DAG.pdf}
   \caption{The DAG approach to increasing the mining rate.}
   \label{fig:dag}
 \end{figure}
 
 \begin{figure}
   \centering
   \includegraphics[width=0.9\linewidth]{figures/Bitcoin_Decouple.pdf} 
   \caption{Deconstructing the blockchain into transaction blocks, partially ordered proposal blocks arranged by level,  and voter blocks organized in a voter tree. The main chain is selected through voter blocks, which vote among the proposal blocks at each level to select a leader block. For example, at level $3$, block $b$ is elected the leader over block $a$. }  
   \label{fig:deconstruct}
 \end{figure}
 

To increase the mining rate while maintaining security, one line of work in the literature has used more complex fork choice rules and/or added reference links to convert the blocktree into more complex structures such as a directed acyclic graph (DAG). This allows a block to be  confirmed by other blocks that are not necessarily its descendents on a main chain. (Figure \ref{fig:dag}). Examples of such works are \ghost\!\! \cite{ghost}, \inclusive\!\! \cite{inclusive}, \spectre\!\! \cite{spectre}, \phantom\!\!~\cite{phantom} and \conflux\!\! \cite{conflux}. However, as discussed in more details in the related work section, \ghost\!\!, \phantom, and \conflux all have security issues \red{(Technically Ghost and Conflux have security issues for high mining rate)}, and \spectre does not provide total ordering of transactions. It is fair to say that handling a highly forked blocktree is challenging. 


 \begin{figure}
   \centering
   \includegraphics[width=0.9\linewidth]{figures/Prism_main.pdf} 
   \caption{\schemenosp. Throughput, latency and reliability are scaled to the physical limits by increasing the number of transaction blocks and the number of parallel voting chains. }  
   \label{fig:parallelize}
 \end{figure}
 

In this work, we take a different approach. We start by {\em deconstructing} the basic blockchain structure into its atomic functionalities, illustrated in Figure \ref{fig:deconstruct}. The selection of a main chain in a blockchain protocol (e.g., the longest chain in \bitcoin\!\!) can be viewed as electing a leader block among all the blocks at each level of the blocktree, where the level of a block is defined as its distance (in number of blocks) from the genesis block. Blocks in a blockchain then serve three purposes: they elect leaders, they add transactions to the main chain, and they vote for ancestor blocks through parent link relationships.  We explicitly separate these three functionalities by representing the blocktree in a conceptually equivalent form (Figure \ref{fig:parallelize}).
In this representation, blocks are divided into three types: proposer blocks, transaction blocks and voter blocks.
The voter blocks vote for transactions indirectly by voting for proposer blocks, which in turn link to transaction blocks . Proposer blocks are grouped according to their level in the original blocktree, and each voter blocktree votes among the proposer blocks at the same level to select a leader block among them. The elected leader blocks can then bring in the transactions to form the final ledger.
The voter blocks are organized in their own blocktrees, which are connected through parent links. Thus, the parent links in the original blocktree have two implicit functionalities which are explicitly separated in this representation: 1) they provide a partial ordering of the proposal blocks according to their levels, and 2) they allow blocks to vote for each other. 
% they help the voting blocks to vote for each other.
%%\red{It's unclear here what is meant by having a block ``support" another block.}



 
This alternative representation of the traditional blockchain, although seemingly more complex than the original blockchain representation, provides a natural path for scaling the performance of blockchain protocols to approach physical limits (Figure \ref{fig:parallelize}). To increase the transaction throughput, one can simply increase the number of transaction blocks that a proposer block points to without compromising the security of the blockchain. This number is limited only by the physical capacity of the underlying communication network. To provide fast confirmation, one can increase the number of parallel voting trees, with many voters voting on the proposal blocks in parallel, until reaching the physical limit of confirming with speed-of-light latency and extremely high reliability. Note that even though the overall  block generation rate has increased tremendously,  the number of proposal blocks per level remains small and manageable, and the voting blocks are organized into many separate voting chains with low block mining rate per chain and hence little forking.  The overall structure, comprising of the three kinds of blocks and the links between them, is a DAG, but a structured DAG.

This complexity management presupposes a way to provide {\em sortition} in the mining process: when miners mine for blocks, they should not know in advance whether the block will become a proposal block, a transaction block, or a voting block, and if it is a voting block, it should not know in advance what particular chain the voting block will be in. Otherwise an adversary can focus its hashing power to attack a particular part of the structure. This sortition can be accomplished by using the random hash value when a block is successfully mined; this is similar to the 2-for-1 PoW technique used in \cite{backbone}, which is also used in \fruitchains\!\!~\cite{fruitchains} for the purpose of providing fairness in rewards. In fact, the principle of {\em decoupling} functionalities of the blockchain, central to our approach, has already been applied in \fruitchainsnosp, as well as other works such as \bitcoinNGnosp. This line of work will be discussed in depth in Section \ref{sec:related}, but its focus is only on decoupling the transactions-carrying functionality. In our work, we broaden this principle to decouple {\em all} functionalities.


 
In \bitcoin\!\!, the irreversibility of a block in the longest chain is achieved by a {\em law of large numbers} effect: the chance that an adversary with less that $50\%$ hashing power can grow a private chain without the block and longer than the public chain diminishes with the depth of the block in the public chain. This is the essence of the random walk analysis in Nakamoto's original paper \cite{bitcoin} and is also implicit in the formal security analysis of \bitcoin in \cite{backbone} (through the definition of {\em typical execution}). The law of large numbers allows the averaging of the randomness of the mining process, so that the chance of the adversary getting lucky and mining many blocks in quick succession is small. This averaging is achieved over time, and comes at the expense of long latency, which increases with the desired level of reliability. 

\scheme also exploits the law of large numbers, but over the number of parallel voter trees instead of over time. Due to the sortition mechanism, the mining processes of both the adversary and the honest nodes are independent across the voting trees. By having many such trees,  many votes are cast on the proposer blocks at a given level, and the chance of an adversary with less than $50\%$ hashing power being able to reverse many of these votes decreases exponentially with $m$, the number of voter trees. The number of voter trees is $m$, and hence the rate of vote generation, is limited only by the physical capacity $C$ of the network. Thus, we can attain irreversibility of a large fraction of the votes with high probability (approaching $1$ exponentially fast in the bandwidth-delay product $CD/B_v$) without waiting for a long time. 
%%	\red{Typo? I think We mean, `Thus we can quickly achieve irreversibility with \emph{high} probability, growing %%exponentially in the bandwidth-delay product $CD$.}
We show that this irreversibility of votes allows fast confirmation of a final leader block  among a list of proposer blocks at a given level. 
In particular, it is guaranteed that the adversary cannot propose another block in the future that has enough votes to become the final leader block at that level. The ability to do this for all levels up to a given level generates  a list of transaction ledgers, one of which must be a prefix of the eventual totally-ordered ledger (Figure \ref{fig:list_decoding}).  
Together with liveness of honest transactions, we show that this ``list decoding" capability is sufficient for fast confirmation of all honest transactions\footnote{List decoding is a concept in coding theory. Instead of decoding to a unique codeword, list decoding generates a list of possible codewords which is guaranteed to contain the true codeword.} in worst case. 
%If one block stands out in terms of number of votes cast  on the different blocks, then the list narrows to this single block, which can then be declared as the leader block. 
If  a given block obtains a substantial enough majority of votes, then the list can be narrowed to contain only that block, which can then be declared the leader block. 
In the worst case, when votes are tied between two or more proposer blocks at the same level (due to active intervention by the adversary, for example),  the irreversibility of {\em all} of the votes and a content-dependent tie-breaking rule is needed to come to  global consensus on a unique leader block;  this requires higher latency. Hence, \scheme requires high latency in the worst case  to guarantee total ordering of all transactions.

\begin{figure}
   \includegraphics[width=.9\linewidth]{figures/List-Ledger.pdf}
   \caption{List ledger confirmation. An example where one can fast-confirm that the final ledger is one of three possibilities. Honest transactions that appear in all three ledgers can be fast-confirmed. Double spends cannot appear in all ledgers and are therefore not fast-confirmed, although one of them will be slow-confirmed.}
   \label{fig:list_decoding}
 \end{figure}
 
The above discussion gives some intuition behind \schemenosp, but a formal analysis is needed to rigorously establish security, latency and throughput performance guarantees. Such a formal analysis was done on \bitcoin in \cite{backbone} in a synchronous round-by-round model and subsequently extended in \cite{pss16} to an asynchronous model with an upper bound on block network delay. In particular, \cite{backbone} pioneered the backbone protocol analysis framework where it was shown that two key properties, the common-prefix property and the chain-quality property, of the \bitcoin backbone guarantee persistence and liveness of the ledger maintained by \bitcoin respectively. We leverage this framework to provide a formal analysis of \scheme in the synchronous round-by-round model (we conjecture that similar results can be established in the more sophisticated asynchronous model of \cite{pss16}). Technically, the most challenging part of the analysis is on fast latency confirmation, where we show that:  1)  the common-prefix property of the voter trees guarantee {\em vote persistence}, so that a large fraction of the votes will not be reversed; 2) the chain-quality of the main chains of the voter trees guarantee vote liveness, so that a large fraction of the voter trees will contain honest  votes on the proposer blocks at each level of the proposal tree.    













==> Eurocryptresponse.tex <==


\section{Eurocrypt Response}


% \subsection{Summary}
% This paper proposes a new PoW-based blockchain protocol that is claimed to
% have much better throughput and latency than existing protocols. At a very
% high level, the protocol splits blocks into three types: proposers, voters and
% transactions. The proposers point to transactions; each proposer has a
% "level", and a single proposer will be the "leader" for each level. The
% leaders determine the ordering of the transaction. Voter blocks vote on the
% proposers; voters are mined in "m" independent blockchains, and each  chains
% gets a single vote per level (the vote of the earliest voter in the chain).
% The leader is the proposer that has the most votes out of the m possible
% votes.

% While there are some interesting ideas here, I'm not convinced the protocol
% actually works, or that the analysis is sound (see "Detailed comments").

\subsection{Reviewer 1}
\textbf{Q:} It appears that there's a "balancing" attack against your Prism protocol (or
perhaps I didn't understand it fully): Suppose there are 3 proposers at level
i; then it could happen that the m voting trees split their votes equally
between two of the proposers, with the remainder going to the third (in case m
is odd). Now no proposer will ever have a majority of the votes. How do you
decide on the leader for level i in this case?

\textbf{A:} In this case a content dependent tie-breaking rule is used:  the proposer block with the smaller hash value will be the leader block. (This is mentioned on the first paragraph in p. 8 of the manuscript.)  Note that the important issue is not that there is a tie in the number of votes, but that the number of votes on each proposer blocks will eventually not change because the votes will become eventually irreversible as they get secured by the voter chains.. This is in contrast to, for example, the situation in GHOST, where the adversary can use saved up blocks from many levels earlier to change the weights (votes) of the subtrees in perpetuity and prevent consensus. Thus, GHOST is vulnerable to a balancing attack and Prism is not. 

\textbf{Q:} It's not clear to me that storing pointers to transactions rather than
transactions themselves can help increase throughput. If you consider a block
valid even if you haven't received the transactions it points to, then you
allow a history-changing attack: an adversary can publish a block with only
the hash of a transaction, but not publish the transaction itself. At some
future date, it can then publish the transaction, which would be valid because
it's already included in an (old) block. On the other hand, if you do require
all of the referenced transactions to be received before you consider a block
valid, you haven't actually gained anything by using a pointer (except when
the same transaction is included in multiple blocks, which isn't where the
throughput improvements come in).


\textbf{A:} In Prism 1.0, we require the transactions blocks to be received before the core block (referring to the tx blocks) is considered valid by a miner; this was not clearly spelled out in the submitted version of the paper and will be added in the revised version. The key point here is that the referred transaction blocks were already transmitted through the network before the core block was mined and hence every honest node will have the transaction blocks before the core block is received. Thus requiring that all the reference transaction blocks to be received does not require any additional delay. 


Here we elaborate on this point a bit further. In section 4.3, the total rate of mining is $f = f_c+f_t$, and in our design we keep $f_c$ small whereas $f_t$ is high. If we had a longest-chain protocol operating at rate $f_c+f_t$, this will lead to a lot of forking and decreased security. However, in Prism 1.0, by separating out the two parts, only the core blocks being produced at $f_c$ are operating using a longest chain protocol - and the forking is minimal. The transaction blocks are produced at a high rate $f_t$ but do not require a linear structure for security on its own, since it is supported by the referencing in the core blocks. 


\textbf{Q:} Using the "bandwidth-delay product" to bound throughput assumes that voting
blocks always include transactions. Why is this necessary? The voting blocks
could, conceivably. include only the nonce and a pointer to a tree of
transactions, so that the "voting rate" is much higher than transaction rate.

\textbf{A:} In the manuscript, we use the bandwidth delay product, measured in number of transactions, to bound the voting rate. This is based on the assumption that the minimum size of a voter block is the size of one transaction. We agree with the reviewer that this is conceptually not correct. Rather the voter block should minimally contain the nonce, parent link and the reference link to the proposer block it is voting on. We will make this point clear in the revision. In practice, however, this minimal size is comparable to the size of one transaction, so the back of the envelope calculations we did on the bandwidth delay product remains reasonable.

\textbf{Q:} More generally, the claim that $(1-\beta)C$ is the best possible throughput
is not convincing; even in your model, where transactions are part of blocks,
what prevents honest blocks from increasing their size if the network capacity
isn't saturated (e.g., if the adversary stops generating blocks)? Conversely,
a malicious adversary might be able to saturate the network with bogus
transactions without generating blocks at all, so it's not clear that
$(1-\beta)C $ is  achievable against a DDoS-ing adversary.

\textbf{A:} The performance measures in the paper, throughput and latency, are worst case measures, worst case in the behavior of the adversary. (See for example the first sentence of Section 4 on p. 13.)  So $(1- \beta) C$ is the worst-case throughput achieved by Prism, worst case when the adversary mine transaction blocks at full rate but fill those blocks with junk transactions.  The actual throughput achieved, however,  can be larger than (1-beta)C. Concerning the second point, we do not model DDoS in this work. In practice, like in Bitcoin, the network imposes a minimum transaction fee to defend against DDos-ing via transaction.

\textbf{Q:} In the description of Prism 1.0, you don't actually specify how the
transaction order is determined (I assume it's using the longest chain of core
blocks?)

\textbf{A:} Yes. That is correct.
















\subsection{Reviewer 2}
% This paper proposes a new blockchain algorithm. The proposed algorithm is
% based on the proofs of work (PoWs), and is using the assumption that the
% majority of the computing power in the system is controlled by honest
% participants. The main idea of the authors is to separate different tasks in
% the blockchain algorithm, by defining 3 types of blocks: “proposer
% blocks”, “transaction blocks” and “voter blocks”. The advantage of
% the proposed solution is that it is more efficient than the original
% Nakamoto’s proposal.

\textbf{Q:} The formal
cryptographic model is not fully defined (e.g. it is not clear how the PoWs
are modelled). As a consequence, the theorem statements miss several important
security assumptions, like: existence of signature schemes or random oracle
model.

\textbf{A:}
We build upon previous work done in modeling the proof-of-work blockchain process in “the bitcoin backbone protocol” paper [5]. There, the hash function for obtaining the proof-of-work is modeled by a random oracle. We utilize the same model in our paper. Furthermore, as stated in that paper, we assume that the digital signature is existentially unforgeable. Finally, in that paper, it has been shown that other error modes in building the blockchain, for example, the probability that two blocks have the same hash, have an exceedingly low probability, exponentially decreasing in the length of the hash function output. Thus we omit a detailed description of these aspects, and instead (1) model the mining by a random process, (2) assume signature schemes are unforgeable, and (3) assume that it is impossible to obtain blocks that match the hash of an existing block. This lets us concentrate on the complementary aspects of the problem, the structure of how the blockchain algorithm works, which is the main contribution of our paper. 

\textbf{Q:} What puzzles me also is the authors’’ statement that “Bitcoin is secure
up to the adversary having 50% of the hashing power of the network nodes”
(on page 2), since it has already been shown by Eyal and Sirer that this is
not true (the authors actually seem to be aware of this paper, since they cite
it [3]). This naturally brings the followiing question to my mind: does the
attack of [3] also apply to the protocol in the paper under submission? It’s
unfortunate that the authors do not address it. 



\textbf{A:} As we mentioned earlier, we build on the “Bitcoin backbone protocol” paper , which models users into two categories: honest and adversarial. The honest nodes follow the protocol exactly whereas adversarial nodes can act arbitrarily within their action space (for example, mining block with arbitrary content, as well as mining on top of arbitrary blocks, as well as revealing these blocks in an arbitrary schedule). In this formal model, the previous paper [5] showed that bitcoin is secure when the adversaries control less than 50% of the hashing power. 

The paper of Eyal and Sirer [3] demonstrated the selfish mining attack where an adversary can get rewards disproportional to the hashing power controlled by the node. Thus, the selfish-mining-attack disrupts fairness but not security. In our model, rewards are not modeled since the users fall into two types: honest or adversarial. The incentive structure is important when users are rational and selfish. Indeed a later algorithm called Fruitchains [14] showed how to defend against the selfish mining attack. This algorithm ensures that each user gets reward (almost) proportional to the hashing power, and thus there is no selfish mining attack possible. We note that our algorithm also has the same property, but we have not emphasized this in the context of the present model.




The paper has also some formatting problems (see pages 14 and 17).
We apologize for the formatting issues and will ensure this is taken care of in the revised version of the paper.















\subsection{Reviewer 3}
\textbf{Summary:}
The paper attempts to construct a proof-of-work blockchain protocol, Prism,
that achieves the physically optimal throughput and latency. This is done by
separating the different functions of the consensus mechanism. The authors
divide the roles of PoW consensus into three
categories: Transaction validation, block proposal and history selection. The
authors claim that decoupling the first from the other two allows for optimal
throughput, separating the latter two allows for optimal latency. In order to
do this, the authors create three distinct blocks (transaction, proposer and
voter) that are mined simultaneously through cryptographic sortition, meaning
that a party cannot predict the type of block which they will mine. The
authors first separate transaction blocks from the main blockchain (Prism
1.0). This allows the protocol to raise the throughput by adding more
transactions to the blockchain without affecting the chain construction. Then,
they separate the blockchain creation in two processes, linked voting blocks
and which vote on proposal blocks which are not directly chained (Prism). This
construction reduces latency for honest transactions by quickly confirming a
set of possible ledgers, under the assumption that all of them will contain
all non double-spent transactions.

Not directly encoding transactions in the blockchain ledger to increase
throughput is a well-studied problem, although never with the goal of finding
the optimal construction. Recent designs have turned towards optimistic
settings in order to deal with confirmation latency. In contrast with systems
like Thunderella, cited by the authors, Prism optimism falls on the honesty of
a transaction: if there is no double spend then the transaction will be
confirmed quickly. This approach is interesting, as it rewards correct
behaviour. This system differs from previous honest-liveness protocols like
SPECTRE and Avalanche in that Prism will eventually create a fully-ordered
log, which will contain one of the double-spent transactions.

\textbf{Q :} While the general structure is explained in an understandable way, the
analysis of the security properties is not. The analysis of Prism 1.0 feels
incomplete, in particular the claim in Section 4.3 that the security of Prism
1.0 is "clearly" the same to the security of Bitcoin.

\textbf{A :} We will be more careful on this point in the revised version.

 More importantly, the analysis for Prism starting in Page 21 is hard to follow
and lacks an explanation of the intuition. The lack of proofs (or intuitive
explanation) for most of the lemmas make it impossible to determine exactly
what is going on. A big problem is the lack of explanation of the choice and
meaning of certain parameters. In the text, the paper claims that the number
of voter chains (m) should be maximized for better security (up to CD, page 7)
but no Theorem or Lemma (including the main result in Theorem 1) includes m.


For example, Theorem 2 mentions m in the preconditions but provides an
equation independent of m. Therefore, it is not clear why it is important to
have a large m. It then seems that the system would be better with m=1, as it
requires less communication and storage. The idea that multiple voting chains
will induce multiple possible ledgers with a common intersection is not
connected with the work that happens in this section. In particular, the
parameter delta is introduced in page 23 as a fraction of the total voting
chains, but why it is necessary or what it represents is never explained.
Going back to Theorem 2, it is trivial to prove that it holds when d=1/2.
Then, in page 26 it is mentioned matter-of-factly that $delta=m^{-0.33}$ with no
prior explanation or justification (and is never mentioned again). This makes
it impossible to effectively judge the value of this paper. For this reason,
we believe this paper cannot be accepted.

\textbf{A :} We apologize that this part of the manuscript was written in a big rush and there are a lot of inconsistencies. We now have a much better version on arxiv but we fully understand that our submission is judged on the submitted version.


\textbf{Q :} It seems that, given a large m, an adversary can perform a double spending
attack as long as a small percentage of voter chains are rewritable and the
adversary can induce a temporary network partition.
The idea is simple, at round r the adversary issues a double spent transaction
t to half of the network and the contradicting transaction
$t^*$ to the other half. Assuming these two halves cannot communicate with each
other, each half will eventually propose a block containing their transaction
and vote on it. After a couple of rounds, both halves of the network
communicate which means that eventually the voting chains should be rewritten
such that almost half of them vote for t and the others vote for $t^*$. One of
the two transactions will have the majority of the votes and therefore be
accepted, wlog lets assume it is t. Then the adversary could possibly rewrite
enough chains to flip the vote to $t^*$, as the number of chains that should be
rewritten should be small as around half of the chains should be voting for
$t^*$ already. Is this the case or is this a consequence of a misunderstanding
of theorem 2?


\textbf{A :}
To confirm a leader block, it should have majority of *permanent* votes. Consider a proposer block with 800 votes of the (say) 1000 total votes. In a case where each of these votes can be removed by the adversary wp 0.5, the proposer block is not confirmed as a leader block because in future that proposer block might have only 800*0.5=400 votes. However in an alternate case, where each vote can be removed w.p .2, the proposer block can be confirmed as a leader block because whp the proposer block will have at least 800*.8 = 640 votes.

\textbf{Q :} You claim that this reaches optimal throughput based on the network delay
B/C+D, however, doesn't the protocol make C grow by creating blocks with a lot
of unnecessary data (as all blocks must simultaneously be valid transaction,
voting and proposer blocks)?  It feels that throughput will be wasted by
having bloated blocks. On the other hand, this would be easy to solve by
having the blocks be represented as Merkle trees (for the purpose of PoW)
where transactions, pointers and votes for distinct subtrees. Then, in the
case a block ends up being a proposer block, in stead of adding the
transactions, only the Merkle root of the transaction tree is added to the
block and communicated (same with votes).

\textbf{A :} We agree. This is included in the revised version.


==> Model.tex <==
\section{Model}
\label{sec:model}

%%In this section, we present a model of \scheme for the analysis in the following section.

\subsection{Mining and communication model}

Let $\N$ denote the set of participating nodes in the network. Each transaction is a cryptographically secure payment message. 
When a transaction arrives at the network, we assume it is instantaneously broadcast to all nodes without consuming any network capacity. We build upon previous work \cite{backbone}, where, (a) the hash function for obtaining the PoW is modeled by a random oracle, (b) the signatures are assumed to be unforgeable, and (c) it has been shown that that the probability that two blocks have the same hash is exponentially decreasing in the length of the hash function output. We make similar assumptions, but concentrate upon the complementary aspects of the problem,  i.e., the structure of the blockchain algorithm design. 
%%\footnote{We assume transaction broadcast does not consume any network resources. However, extending the model to include the cost of transaction propagation %%is an interesting direction for future work.}
%%A \textit{block} consists of an ordered list of $B$ transactions and a few reference links to other blocks. 
Each  node $n\in \N$ controls $p_n$ fraction of total hashing power and it mines blocks according to Algorithm \ref{alg:prism_minining}. We model the node's aggregate block generation process by a Poisson process with rate $fp_n$ blocks per second, further split via the sortition process into independent Poisson processes with rates $f_p p_n$, $f_t p_n$ and $mf_vp_n$ for proposer, transaction blocks and voter blocks respectively. The voter blocks are further split into independent Poisson processes with rate $f_vp_n$, one for each of the $m$ voter chains. 

There are two types of nodes -- honest nodes, $\H\subset \N$, who strictly follow the protocol, and the adversarial nodes, $\N \setminus \H$, who are allowed to not follow the protocol.
The adversarial nodes control $\beta$ fraction of hashing power i.e, $\sum_{n\in \N/\H}p_n=\beta$, whereas the honest nodes control the other $1-\beta$ fraction of hashing power\footnote{$\beta$ for {\bf b}ad.}. As a consequence, the honest nodes mine blocks with overall Poisson process rate $\sum_{n\in \H}fp_n = (1-\beta)f$ and the adversarial nodes mine blocks with Poisson process rate $\sum_{n\in \N \setminus\H}fp_v = \beta f$. Without loss of generality we can assume a single adversarial node with $\beta$ fraction of hashing power. Note that while an adversary does not need to follow protocol and can, for example, not mine on the longest chain, the split of the aggregate mining process into the individual processes for the three types of blocks holds regardless of whether a node is honest or adversarial, since adversaries cannot control the sortition process.
%%We will also assume that the number of honest nodes is large and the fraction of hashing power each node has is correspondingly small.

The nodes exchange blocks  via a broadcast channel. The time taken transmitting a block from one honest node to another honest node is assumed to be $\Delta$ seconds.  On the other hand, the adversary can transmit and receive blocks with arbitrary delay, up to delay $\Delta$.

To simplify our analysis, we discretize the above continuous-time model into the discrete-time round-by-round synchronous model proposed in \cite{backbone}. Each round in this model corresponds to a time interval of $\Delta$ seconds in the continuous-time model above, and the number of blocks generated by each process in that round is the number of blocks generated over that time interview. Let $H_i[r]$ and $Z_i[r]$ be the number of voter blocks mined by the honest nodes and by the adversarial node in round $r$ on the $i$-th voting tree respectively, where $i=1,2,..,m$.  $H_i[r], Z_i[r]$ are Poisson random variables with means $(1-\beta)f_v\Delta$ and $\beta f_v \Delta$ respectively. Similarly, $H^p[r], Z^p[r]$ are the numbers of proposer blocks mined by the honest nodes and by the adversarial node in round $r$ respectively; they are also Poisson, with means $(1-\beta)f_p\Delta$ and $\beta f_p \Delta$ respectively. Finally, $H^t[r], Z^t[r]$ are the numbers of transaction blocks mined by the honest nodes and by the adversarial node in round $r$ respectively; they are also Poisson, with means $(1-\beta)f_t \Delta$ and $\beta f_t \Delta$ respectively. All the random variables are independent of each other. 

%%For the honest nodes, we define $X_i[r]$ $( X^p[r])$, which is $1$ if $H_i[r]\ge 1$ $(H^p[r] \ge 1)$ and zero otherwise. and define $Y_i[r]$ $( Y^p[r])$, which is $1$ if $H_i[r]=1$ $(H^p[r] = 1)$ and zero otherwise. The variables $Y_i[r]$ and $Y_p[r]$ are analogous to  the  random variable defined in \cite{backbone} to indicate whether the $r$th round is a {\em uniquely successful} round, i.e. a round in which only one block is mined by the honest nodes .
%% We denote  $H_i[r_1, r_2] := \sum_{r=r_1+1}^{r_2} H_i[r]$, similarly for $Z_i,X_i$ and $Y_i$. The interval $[r_1, r_2]$ denotes rounds $\{r_1+1,r_1+2,\cdots,r_2-1,r_2\}$.

Honest nodes follow the \scheme protocol (Algo \ref{alg:prism_minining}).  The honest blocks are immediately broadcast  to all the nodes during the round they are mined. The adversary may choose to keep some or all of the  blocks  they mined private. The adversary may also choose to broadcast any private block it mined from previous rounds. The adversary is allowed to first observe the blocks honest nodes mined in a round and then take its action for that round.
 It can also decide which longest chain each honest node mines on (if there are more than one), and which proposer block each honest voter votes on (but it cannot remove the vote or violate protocol, e.g., by changing the proposal block level of the vote.)  The adversary is powerful as it can observe what is happening in {\em all} the trees to make a decision on its action in any individual tree. In particular, this adversarial power means that the evolution of the trees can be {\em correlated} even though the mining processes on the different trees are independent (because of the sortition procedure). This fact makes the analysis of \scheme more subtle, as we need to prove some kind of law of large numbers across the voter trees, but can no longer assume independence.
We assume all the nodes have a common view of the (public) trees at the end of each round.

Following the \bitcoin backbone protocol model \cite{backbone}, we consider protocols that execute for a finite number of  rounds, $\rmax$ which we call the execution horizon.  We note that we do not consider cryptographic failure events, such as insertion in the blockchain, since it has been demonstrated in the backbone protocol paper that for a polynomial number of rounds $\rmax$ in the hash-length, these events have negligible probability. 
\vspace{-3mm}
\subsection{Network model}
To connect to the physical parameters of the network, we assume a very simple network model. Let $B_t$, $B_v$ and $B_p$ be the size of a transaction-, voter- and proposer block respectively,  in units of number of transactions. The network delays $\Delta_t,\Delta_v$ and $\Delta_p$ for each type of blocks is given by:
\begin{equation} 
\label{eq:delay}
\Delta_t  = \frac{B_t}{C} + D, \quad \Delta_v  = \frac{B_v}{C} + D,  \quad \Delta_p  = \frac{B_p}{C} + D
 \end{equation}
i.e. there is a processing delay of $B/C$ followed by a propagation delay of $D$ seconds.  This is the same model used in \cite{ghost}, based on empirical data in \cite{decker}, as well in \cite{subchains}. However, here, we put an additional qualification: this expression is valid only assuming the network is stable, i.e. the total workload of communicating the blocks is less than the network capacity. In terms of our parameters:
\begin{equation}
f_p B_p + m f_v B_v + f_t B_c < C.
\label{eq:stability}
\end{equation}
For a given block size, \eqref{eq:stability} imposes a physical constraint on the total mining rate $f$.
This \emph{stability constraint} sets our model apart from prior work, which has traditionally assumed infinite network capacity; in particular, this gives us a foothold for quantifying physical limits on throughput and latency.

Given that different types of blocks have different sizes and have different network delays, what is a reasonable choice for $\Delta$, the duration of a round in the synchronous model? Since the synchronous model is used for security analysis, and the security of \scheme depends only on the network delay of the proposer and voter blocks but not of the transaction blocks, we choose:
$$ \Delta = \max \{ \Delta_p, \Delta_v\}.$$
 
 %%Since transaction blocks are typically larger than the other two types of blocks (which contain only reference links), this model essentially speeds up the communication of transaction blocks, but the security of the protocol is not affected. 


%%Note that the protocols discussed in this manuscript can be used in any network setting. This simple network model is only used as a common baseline to evaluate how well a particular 
%%protocol performs relative to the physical limits. In particular, the delay model \eqref{eq:delay} ignores queuing delay due to randomness of the times of the block transmission across the network. 

%%\red{Did we decide not to include precise definitions of our metrics? I think we should eventually have a 3rd subsection where we do this}  They are implicit in the analysis and theorems.



%%\begin{itemize}
%%    \item Continuous time
%%    \item Ghost attack
%%    \item Scheme - Coloring and Scheduling.
%%    \item Proof (Continuous time)
%%\end{itemize} 

==> analyze_others.tex <==

\section{Throughput Analysis of GHOST}

First, we compute the growth rate of the main chain, assuming pessimistically only honest users work on it. Blocks are mined by the honest nodes, and the times at which they are mined follow a Poisson process  at rate $(1- \beta) f$. The mining is done  on the main chain as given by the GHOST rule, computing the main chain always by branching to the subtree with the largest number of blocks \cite{SZ13}. Once a node mines a block, it broadcasts the block to the rest of the network and whenever nodes receive the block they append it to their current view of the tree. The growth rate of the main chain is the rate at which blocks are added on top of each other at a node, and is given by the following lemma (Lemma 6 of \cite{SZ13})

\begin{lemma}
(\cite{SZ13}) The growth rate of the main chain under the GHOST rule  is at least 
\beq
\frac{(1-\beta)f}{1 + 2(1-\beta)f\Delta} \quad \mbox{blocks per second.}
\eeq
This lower bound is tight in the case when the number of nodes is large and the compute power is split evenly between the nodes.
\end{lemma}

An observation is that the throughput increases monotonically with the PoW rate $f$. The GHOST rule has the property that for any $\beta < 0.5$ and for any $f$, the system is secure. This means we should increase $f$ as much possible. However, $f$ is bounded by the stability constraint \rref{eq:stability}. Hence the throughput is maximized by setting:
\beq
 f^*_{\rm GHOST} = \frac{C}{B},
 \eeq
leading to a throughput of 
\beq
\frac{\lambda}{C} = \frac{(1-\beta)}{1+2(1-\beta)(1+\frac{C}{B}D)}
\eeq
The quantity
\beq \frac{C}{B} \cdot D
\eeq
is analogous to the concept of {\em bandwidth-delay product} in networking, where bandwidth is measured in terms of number of blocks per second the network can transport. It can be thought of as the number of blocks "in flight". The above expression says that the throughput is monotonically decreasing with this quantity. So to maximize the throughput, we should may this bandwidth-delay product should be made as small as possible, by letting the block size $B$ large. Indeed, by setting $B$ such that :
\beq
 \frac{C}{B} \cdot D \ll 1,
 \eeq
we achieve the maximum throughput:
\beq
 \frac{\lambda^*_{\rm GHOST}}{C} = \frac{1-\beta}{3 - 2 \beta}.
 \eeq

\section{Comparison with throughput of Bitcoin}

We can compare this throughput to the maximum achieve throughput for Bitcoin. Unlike GHOST, Bitcoin adopts the longest chain strategy: the miners always work on the longest chain in their view of the block tree. The growth rate of the longest chain is given by Lemma 5 in \cite{SZ13}:

\begin{lemma}
(\cite{SZ13}) The growth rate of the longest chain under the " mine the longest chain" rule is at least 
\beq
 \frac{(1-\beta)f}{1 + (1-\beta)f\Delta} \quad \mbox{blocks per second.}
 \
 \eeq
This lower bound is tight in the case when the number of nodes is large and the compute power is split evenly between the nodes.
\end{lemma}

Just as in the GHOST rule, the throughput of Bitcoin increases monotonically with the PoW rate $f$.  However, in addition to the stability constraint \rref{eq:stability}, there is a {\em security} constraint on $f$ as well. Because the security provided by Bitcoin solely rests on the length of the longest chain (as opposed to GHOST, which is based on the number of blocks in the entire honest subtree), we must make sure that $f$is chosen such that the growth rate of the longest honest chain is larger than the growth rate an adversary chain. This leads to the following condition on $f$:
\beq
 \frac{(1-\beta)f}{1 + (1-\beta)f\Delta}  > \beta f.
 \label{eq:security}
 \eeq
 The left hand side is the growth rate of the longest honest chain. The right hand side is the most optimistic growth rate of an adversary chain: blocks are built on top of each other without network delay. Since we are performing a worst case security condition, we need to assume the fastest possible adversary growth rate. 

Eq. \rref{eq:security} leads to the following upper bound on $f$:
\beq
f \Delta < \frac{1-2\beta}{\beta(1-\beta)}. 
\eeq
 Combining this with the stability constraint, we should choose the best $f$ for Bitcoin as:
 \beq
 f^*_{\rm BC} \Delta = \min \left (  \frac{1-2\beta}{\beta(1-\beta)}, 1 + \frac{C}{B} \cdot D \right ).
\eeq

There are now two possibilities:

\begin{enumerate}
\item  If 
\beq
\frac{1-2\beta}{\beta(1-\beta)} < 1
\eeq
or equivalently, $\beta > \frac{3-\sqrt{5}}{2}$,  then, optimizing over $B$ yields 
\beq
\frac{\lambda^*_{\rm BC}}{C} = \frac{1-2\beta}{1- \beta}. \label{eqn:bc_thruput_small_beta}
\eeq
 \item On the other hand if $\beta <  \frac{3-\sqrt{5}}{2}$, then 
 \beq
\frac{\lambda^*_{\rm BC}}{C} = \frac{1-\beta}{2- \beta}. \label{eqn:bc_thruput_large_beta}
\eeq
\end{enumerate}

The throughputs of GHOST vs Bitcoin are plotted in Figure \ref{fig:thruput}

\begin{figure}
\hspace*{-2.4cm}                                                           
  \includegraphics[scale=.95]{Picture1.png}
  \caption{(a) Maximum throughput vs $\beta$ Adversarial power - for fixed $\epsilon$ and no constraints on latency. The thruput for Bitcoin protocol exhibits a change at $\beta= \frac{3-\sqrt{5}}{2}$, as per equations \eqref{eqn:bc_thruput_small_beta} and \eqref{eqn:bc_thruput_large_beta}. 
  (b) Latency vs $\beta$  for fixed $\epsilon$ and no constraints on thruput. Ghost$++$ out performs Bitcoin because it uses heaviest subtree decoder instead of longest chain decoder.
  (c) Latency vs $\ln\big(\frac{1}{\epsilon}\big)$ for fixed $\beta$ and no constraints on thruput.
  (b) Latency vs thruput for fixed $\beta$ and fixed $\epsilon$. Bitcoin protocol changes its behaviour at $\beta= \frac{3-\sqrt{5}}{2}$, as per equations \eqref{eqn:bc_thruput_small_beta} and \eqref{eqn:bc_thruput_large_beta}.}
\end{figure}



\section{Latency of GHOST++}

For a given block size (i.e. given network delay $\Delta$), the confirmation latency is minimized by choosing the largest possible $f$. For GHOST++, the largest $f$ is also the same as the one that maximizes the throughput, i.e.
\beq
 f^*_{\rm GHOST++} = \frac{C}{B},
 \eeq
 The quantity 
 \beq
 f^*_{\rm GHOST++} \Delta = 1 + \frac{C}{B} \cdot D
 \eeq
 is the expected number of blocks mined during the time interval $\Delta$, and it is a measure of how close the system can be approximated by a fluid model over the time scale $\Delta$. If 
 \beq
 f^*_{\rm GHOST++} \Delta \gg 1,
 \eeq
i.e. the bandwidth delay product
\beq
 \frac{C}{B} \cdot D \gg 1
 \label{eq:bdp}
 \eeq
 then many blocks are mined over this time scale, and we can regard the honest nodes as well as the adversary working at deterministic rate of $(1-\beta)f^*_{\rm GHOST++}$ and $\beta f^*_{\rm GHOST++}$ blocks per second respectively. Under this assumption, the latency $\tau$ that one needs to wait before being sure that the adversary cannot tamper with a transaction (by building a larger subtree than the honest nodes) should satisfy:
 \beq
 \beta f^*_{\rm GHOST++}  \tau < (1- \beta) f^*_{\rm GHOST++} (\tau -\Delta).
 \eeq
 This condition can be interpreted as follows. The left hand side is the amount of work that the adversary can do over a time window $\tau$. The right hand side is the amount of work that the honest nodes can do over the same window, but it's delayed by $\Delta$. This leads to a latency of 
 \beq
\tau = \frac{1-\beta}{1-2 \beta} \Delta
 \eeq
By choosing $B = 1 $ transaction, and since we assume condition \rref{eq:bdp}, we achieve the best latency of :
\beq
\frac{\tau^*_{\rm GHOST++}}{D} = \frac{1-\beta}{1-2\beta}.
\label{eq:latency}
\eeq
Interestingly, $B=1$ also makes the condition \rref{eq:bdp} the easiest to satisfy, hence the choice of $B = 1$ kills two birds with one stone. Moreover, it is conjectured that the latency bound \rref{eq:latency} is in fact the best that can be achieved by {\em any} PoW blockchain scheme.

With this analysis, it is now seen that the physical assumption that is needed to achieve the optimal latency bound \rref{eq:latency} is precisely $C \cdot D \gg 1$, i.e. the bandwidth delay product, i.e. number of {\em transactions} in flight,  is large. It is also interesting to note that while a very large block size (and very small number of blocks in-flight)  is required to achieve the best throughput, a very small block size (and a very large number of blocks in-flight) is required to achieve short latency. The next step is to study the tradeoff between latency and throughput.

\section{Throughput of Conflux}

Recently, a new PoW consensus algorithm called Conflux was invented \cite{conflux18}. Amazingly, it can merge all the blocks in the tree into a unified ledger and it achieves a throughput given by the following lemma.

\begin{lemma}
(\cite{conflux18}) For a given PoW rate, the throughput of Conflux is at least 
\beq
 (1-\beta)f  \quad \mbox{blocks per second.}
 \
 \eeq
This lower bound is tight in the case when only the honest nodes mine blocks.
\end{lemma}

As in GHOST and Bitcoin, the throughput of Conflux increases monotonically with the PoW rate $f$. Conflux shares the GHOST's property that for any $\beta < 0.5$ and for any $f$, the system is secure. This means we should increase $f$ as much possible. However, $f$ is bounded by the stability constraint \rref{eq:stability}. Hence the throughput of is maximized by setting:
\beq
 f^*_{\rm Conflux} = \frac{C}{B},
 \eeq
leading to a throughput of 
\beq
\lambda^*_{\rm Conflux} = (1-\beta) \frac{C}{B} \cdot B \quad \mbox{Tx/second} = (1-\beta) C \quad \mbox{Tx/second} 
\eeq
i.e.
\beq
\frac{\lambda^*_{\rm Conflux}}{C} = 1-\beta
\eeq

Two observations:
\begin{itemize}
\item  This is the optimal throughput achievable by {\em any} decentralized scheme. Power to Yao!

\item  Unlike GHOST, GHOST++ or Bitcoin, the throughput of Conflux does not depend on the network delay $\Delta$. Hence, the throughput of Conflux does not depend on the block size $B$. Recall that in GHOST++, there is a tension between maximizing throughput (large $B$) and minimizing latency (small $B$), thus leading to a tradeoff between latency and throughput. No such tension exists for Conflux. Maximizing throughput does not put any constraint on $B$. Hence, to minimize latency, we should simply choose $B$ as small as possible. Assuming GHOST++ decoder can be used in conjunction with Conflux, one should be able to get the optimal latency and the optimal throughput {\em simultaneously}.
\end{itemize}

 \section{Through and Latency: End-to-end analysis}
 
 The analysis of throughput and latency are incomplete. For example, the analysis of Conflux makes the (overly?)  optimistic assumption that the blocks contain no overlapping transactions so that throughput in terms of blocks per second translate fully to throughput in terms of transactions per second. Moreover, the confirmation latency we calculated is from the time the block got mined to the time when the transaction is confirmed. It ignores the time from the transaction arrival to the time the transaction got into the block. In this section we will do an end-to-end analysis on these two quantities. To do this, we need to model how transactions enter the blocks.
  
 \subsection{Single Transaction Queue}
 
Lets start with a simple case, when transactions arrive at a single queue and nodes takes $B$ transactions at the head of the queue and mine the block simultaneously starting at time $0$. Lets call this block $1$. When one node, say node $i$,  succeeds in mining block $1$, say at time $t$, it will broadcast that block to the rest of the nodes and takes the next $B$ transactions in the queue to mine a new block, block $2$. Other nodes continue mining block 1 until they receive the broadcasted block $1$ from node $i$ after a delay of $\Delta$. Assuming for simplicity that every broadcasted block is subject to the same delay and the delay is the same for every node, the block broadcasted by node $i$ will be the first block received by all other nodes.  Before then, other nodes do not realize that block 1 has been mined already, and some of these nodes may also mine block $1$. There are on the average $(1-\beta) f  \Delta$ such redundant copies of block. These nodes will also go on to mine block 2. At time $t +\Delta$, all the other nodes which are still working on block $1$ will abandon block $1$ (no point since block 1 is already in the tree and will be included in the ledger by Conflux) and move on to block $2$. Assuming the regime where there are many nodes with small compute power, we ignore the event that a  node can be mining block 3 at this point. So at time $t+\Delta$, everybody is mining block 2 and the whole process starts over again.

Hence, the goodput of Conflux (number of distinct blocks generated) is
\beq
\frac{(1-\beta)f}{1 + \Delta f (1-\beta)} \quad \mbox{number of blocks per second}
\eeq
which is identical to the one conjectured to be achieved by GHOST. So in this setting, there is no gain in using Conflux over GHOST.

\subsection{Multiple Transaction Queues}

The problem with the previous scheme is that too many identical blocks are mined at the same time. Let us then distribute the transactions into $m$ queues, and have each node randomly assigned to each queue (a color).  The scheme is the same as before but each node only picks transactions from the head of the queue of its color. This reduces the number of redundant blocks mined by a factor of $m$, and the goodput of Conflux (number of distinct blocks generated) is
\beqa
\lambda & = & \frac{(1-\beta)f}{1 + \frac{1}{m} \Delta f (1-\beta)} \quad \mbox{number of blocks per second}\\
& = &  \frac{(1-\beta)fB}{1 + \frac{1}{m} \Delta f (1-\beta)} \quad \mbox{transactions per second}
\eeqa
Setting 
\beq
f^* = \frac{C}{B}
\eeq
to optimize this, we get:
\beq
\bar{\lambda} = \frac{\lambda}{C} = \frac{m(1-\beta)}{1+\frac{CD}{B} +m}
\eeq
Note that for any $B$, we can achieve the optimal throughput of $\bar{\lambda}^* = 1 -\beta$ by choosing $m \gg 1+\frac{CD}{B}$. So achieving optimal throughput does not constrain $B$. However, since the latency depends on $m$, we can no longer conclude that there is no tradeoff between throughput and latency.

Since we have a degree of freedom in choosing $B$, let us choose $B$ such that 
\beq
1+\frac{CD}{B}  \gg 1.
\eeq
Under this assumption, the network delay $\Delta$ is the propagation delay $D$. The confirmation latency, assuming things work out for the GHOST++  decoder, is
\beq
\frac{1-\beta}{1-2\beta} D
\eeq
However, the end-to-end latency of a transaction is the sum of this confirmation latency and the latency from the time the transaction enters its queue and the first time the transaction enters the blockchain tree (i.e. first time a block containing that transaction is successfully mined.). Let us calculate the latter by considering the dynamics of a transaction queue. Transactions enter this queue at a deterministic rate $\lambda/m$ transactions per second. For stability, they must also be cleared at a rate of $\lambda/m$. Thus it takes time $m B/\lambda$ seconds to clear a block of $B$ transactions from the queue. A block is cleared when every node that is mining the block abandons the block and move on to the next block because they heard that the block has already been mined by some other node. Thus, the first time the block is successfully mined by some node happens $\Delta$ time before that. Ignoring queueing delay, the latency from the time a transaction arrives to the time it is first successfully mined is 
\beq
\frac{mB}{\lambda} - D
\eeq
Hence, the total confirmation latency is:
\beq
\tau = \frac{mB}{\lambda} - D + \frac{1-\beta}{1-2\beta} D
\eeq

We can see the first term increases with $m$ as $\lambda$ approaches the optimal throughput. This suggests we don't want to choose $m$ arbitrarily large. In fact, a natural scaling is to choose $m$ as:
\beq
m = \bar{m} ( 1+\frac{CD}{B} )
\eeq
In terms of $\bar{m}$, we now have the following:
\beqa
\bar{\lambda} &=& \frac{\bar{m}}{\bar{m}+1} (1-\beta)\\
\bar{\tau} & = & \tau/D =  \frac{\bar{m}+1}{1-\beta} - 1 + \frac{1-\beta}{1-2\beta}
\eeqa
Eliminating $\bar{m}$, we have the following tradeoff between $\bar{\tau}$ and $\bar{\lambda}$:
\beq
\bar{\tau}= \frac{\beta+ \bar{\lambda}}{1-\beta-\bar{\lambda}} + \frac{1-\beta}{1-2\beta}
\eeq
 
 This tradeoff is plotted in the figure for $\beta = 0.4$. 
 
 \begin{figure}
                                                          
  \includegraphics[scale=.95]{tradeoff.pdf}
 \caption{Tradeoff between $\bar{\tau}$ and $\bar{\lambda}$ for $\beta = 0.4$.}
 \end{figure}


 Some observations:
 
 \begin{itemize}
 \item There is indeed a tradeoff between throughput and latency. Sreeram is right!
 \item On the other hand, there is indeed no constraint on what block size to get good throughput. So this allows us to get a fraction of the optimal throughput while gettting a constant factor of the min latency independent of $\epsilon$. Bitcoin or GHOST cannot achieve this kind of tradeoff. So indeed Conflux is useful.
 \item Is this the {\em optimal} tradeoff?
 \end{itemize}






 





 
 





==> comments.tex <==
Things to do

1. Need to make sure model contains details about delay model, capacity constraints as well as clock assumptions (synchronous or otherwise)
-> Mention that we do not deal with cryptographic failures, which already backbone showed are negigible for polynomial no of rounds in the hash length. Explain that delay is due to communication but also due to processing. 

2. Explain variables Y and Z in the latency section  or somewhere

3. Incentive compatibility - mention in intro

4. Smart contract - abstract / intro

5. Latency section 
-> Add lemma about when confirmation can happen

-> Add intuition and structure for proof

-> Notation: P_{\ell}(r)

6. Related work - improve

7. Add section on throughput + latency

8. fv vs f - notation

proposer list confirmation policy

==> discussion.tex <==
\section{Discussions}

\label{sec:discussion}

\subsection{\schemenosp: incentives} Our discussion on \scheme has mostly focussed on honest users and adversarial behavior. Here we briefly discuss rational behavior, and the accompanying reward structure that incentivizes rational users to participate in the system without deviating from the proposed protocol. There are straightforward approaches to add a reward structure to \schemenosp. Each block, whether a voter block or a proposal block, that finds its place in the ledger is assigned a block reward. To allocate transaction fees, we follow the method proposed in Fruitchains \cite{fruitchains}. The transaction fees are distributed among the past $Q$ blocks, where $Q$ is a design parameter. In \schemenosp, all blocks eventually find a place in the ledger, and thus the proportion of blocks contributed by a miner to the ledger is proportional to the hash rate of the miner.  For  large values of $Q$, our design ensures that incentives are fairly distributed and there is no gain in pursuing selfish-mining type attacks \cite{sapirshtein2016optimal}. 

{\bf Todo: Add a small para for smart contracts and PoS}

% \subsection{\schemenosp: smart contracts}

% Most of our discussion on \scheme has focused on transactions. However, we point out here that \scheme is not restricted to processing transactions and can be extended to process complex smart contracts. Smart contracts are pieces of code which are executed based on the current state of the ledger. Importantly, they can depend on the {\em history of the ledger}, including on the timing of various events recorded on the ledger. While many of the basic blockchain protocols such as longest-chain consensus or \ghost protocol can accommodate smart contracts, newer schemes  such as \spectre and \avalanche are specific to transactions and do not confirm smart contracts. We note that \scheme is naturally able to confirm the output and final-state of every smart contract at the $\eps$-dependent latency since we get total order. We also note that this is the behavior desired in hybrid algorithms like \phantom + \spectre.

% We note that \scheme has an additional attractive property for smart contracts - the ability to confirm several smart contracts at a short latency (proportional to propagation delay). Since \scheme is able to confirm a list of ledgers within a short latency, this can be exploited to confirm some smart contracts. If a smart contract will execute to the same final state and output in all the ledgers in this list, then this output and final state can be confirmed for the smart contract even before confirming a unique ledger. We recall that \scheme guarantees short confirmation time for honest transactions. Analogous to the notion of honest transactions, we can define a notion of {\em uncontested smart contracts}, where there is no alternate view of how the events happened in any of the blocks. Such uncontested smart contracts can then be shown to be confirmed within a short $\eps$-independent  latency proportional to the propagation delay - thus enhancing the scope and utility of \scheme beyond payment systems.   




% \subsection{\schemenosp: Proof-of-Stake}
% In this paper we have described \scheme in the proof-of-work (PoW) setting that scales the throughput by three orders of magnitude over \bitcoin. Despite this significant increase,  PoW is nevertheless  energy inefficient (\bitcoin consumes as much energy as medium sized countries \cite{de2018bitcoin}) and a leading alternative is the  so-called proof-of-stake (PoS)  paradigm. PoS restricts involvement in the consensus protocol to nodes who deposit a requisite amount of stake, or currency, into the system. This stake is used as a security deposit in case the nodes misbehave -- for instance, by trying to unduly influence the outcome of consensus. PoS is appealing for several reasons, including the fact that it can be much more energy-efficient than PoW and also because it can be  more incentive-compatible. 

% There are two key issues associated with designing a PoS version of \schemenosp. First, a cryptographically secure source of randomness, that is distributed and verifiable, is needed to replace the source of randomness currently used in \scheme -- this includes the various mining steps,  transaction scheduling and sortition operations. Second, PoS does not have the conservation of work that is implicit in PoW and this allows adversaries to ``mine" at no cost in parallel and only report  the outcomes that can be successfully verified -- this exposes new   security vulnerabilities (popularly known as the ``grinding" \cite{grindingwiki} and ``nothing at stake" attacks \cite{li2017securing,kiayias2017ouroboros}) and a PoS design of \scheme will have to contend with this attack. Both these obstacles can be successfully surmounted and will be the topic of a forthcoming paper \cite{prismpos}.  

%%\textit{Randomness source: }In PoW, transactions are the key source of randomness, which cannot be tampered with unlike other parts of the block such as its  metadata.  However,  we cannot use transactions for the source of randomness in PoS since a validator could    take  other step to try to bias the randomness in their own favor, strategies classified in the literature as  grinding attacks \cite{grindingwiki}. A first order solution is to maintain a source of randomness outside the blockchain via multiparty computation,  as suggested in early PoS designs \cite{kiayias2017ouroboros}. However, this design is not scalable (in number of nodes,  transaction rates or over time) and is also against the spirit of the blockchain design principle which seeks to be internally consistent and unreliant on external (random) sources.  
%%Our proposal is to maintain a source of randomness within the blockchain which starts at the genesis block and  evolves along the blocktree using verifiable random functions (VRFs) \cite{david2018ouroboros,gilad2017algorand,li2017securing}. Analogous versions of this  approach have been used in recent PoS designs such as \cite{gilad2017algorand} and  \cite{badertscher2018ouroboros}. 
%%As a result, the mining process in PoW can be mimicked in a PoS blockchain using VRFs  except for nothing at stake attacks, discussed next. 

%%\paragraph{Nothing at stake:} In a PoW blockchain, the adversary has to split its computational resources to mine on different chains. However, in a PoS blockchain using VRFs, the adversary can mine on multiple chains without dividing its stake. As a consequence, the adversary can grow many chains in private and `attacks' using the successfully verifiable longest chain among all these private chains. This is the nothing at stake attack and we analyze it by posing the growth of these multiple chains as a Galton-Watson tree with immortal nodes \cite{shi2015galton}. It turns out that the growth rate of the depth of this tree is equal to the growth rate of the longest private chain. On analyzing these trees, one can show that the adversary's mining power is boosted by a small constant factor, which is equal to  $e$ in a straightforward implementation -- i.e., the longest private chain grows at rate $e\beta$ (instead of $\beta$) \cite{fan2018scalable}. The Galton-Watson tree framework allows us to alter the VRF technique such that growing multiple chain in private will boost the adversary's power only by a factor of $1+o(1)$. As a result, this will translate to security up to $\beta=\frac{1}{2}$.


% \subsection{\scheme\!\!: List ledger decoding vs Unique ledger decoding}

% \scheme provides two ways to confirm transactions -- list ledger decoding and unique ledger decoding. \scheme returns a list of ledgers with constant latency $\tau_{\text{list}}$ (which is independent of $\epsilon$), and a transaction is confirmed if it is recorded in all the ledgers in the list. For example, {\em honest} financial transactions such as ``Alice pays Bob \$10" can be confirmed using this method. Honest transactions do not have competing double-spends and due to a liveness property, such transactions find a place in every ledger in the list in a constant amount of time. We note that our methodology of list-decoding permits us to confirm complex transactions such as smart-contracts in the list decoding phase, as long as there are no competing views and such smart contracts are confirmed in every ledger. 



% The ledger list size (up to a fixed level $\ell$) decreases with time and eventually converges to a unique ledger with latency $\tau_{\text{unique}}$ - this latency is $\eps$-dependent and hence potentially slower. All kinds of transaction (example: smart contracts) will get confirmed on a unique ledger. 
% The confirmation time of a double-spend transaction or a contentious smart-contract ranges from $\tau_{\text{list}}$ to $\tau_{\text{unique}}$ depending on its complexity. We note that in scenarios where there are few adversaries, our list decoding is likely to contain a singleton item within a short amount of time, and all types of transactions and smart contracts can be confirmed. Thus our algorithm provides a natural adaptivity to the fraction of adversary, $\beta$.




==> latency+thruput.tex <==
\subsection{Latency and throughput}

So far we have focused on getting short latency. To simultaneously achieve short latency (on honest transactions) as well as high throughput, we can use the ideas of \schemelite and add reference links from the proposer blocks to the transaction blocks.
See Figure \ref{fig:sortition_structure} for a summary of all the types of blocks and link structure of \scheme.

\begin{figure}
  \centering
  \includegraphics[width=1.1\linewidth]{figures/Sortition.png}
  \caption{Summary of the block structure and the sortition procedure. \label{fig:sortition_structure}}
 \end{figure}

==> latency_prelude.tex <==
\section{Latency analysis}

Confirmation rule
-> List decoding policy


\subsection{Proposer-list confirmation policy} 




Given parameters $\theta,\nu$.

Given a set $P_{\ell}(r) = \{B_1,...,B_P\}$ of proposers at level $\ell$ at round $r$, let the number of votes for proposer block $B_p$ at round $r$ be $v_p(r)$. We calculate a lower-bound $\underbar{v}_p(\cdot)$ on $\overbar{v}_p(\cdot)$ such that  \beq v_p(r') \geq \underbar{v}_p(r) \quad \forall r' \geq r. \eeq  

Let block $B_p$ have $m \times v_p^{ k}(r)$ votes at depth $k$ or greater in the voting trees. Note that for any $k$, $\sum_p v_p^{ k}(r) \leq m$, where $m$ is the number of trees, since each tree can vote only for one of the blocks. 







Let $\{\delta_k, k=0,1,2,...\}$ be a set of parameters specified by the algorithm. Then the lower bound on the number of votes is given by 
\beq 
\underbar{x}_p(r) := \max_{k \geq 0} \{ (v_p^{ k}(r) -\delta_k m)^{+} \}. \eeq


For a given subset of proposer blocks $I \subseteq P_{\ell}(r)$, we can calculate, a lower bound on the total number of votes for this subset as follows

 
\beq  \underbar{v}_I(r) :=  \max_{k \geq 0} \{ (v_I^{ k}(r) -\delta_k m)^{+} \}. \eeq  where $v_I^k(r)$ is the number of trees that voted at-least k-deep for one of the subset $I$.

Now the upper bound on votes at a given time can be stated as follows:

\beq \bar{v}_p(r) = m - \underbar{v}_{p^c}(r), \eeq
where $p^c = P_{\ell}(r) \setminus \{p\}$ is the set of all proposers other than $p$ at the given time. We emphasize that the two values give an upper and lower bound on the number of votes at any given round  - except with probability vanishingly small in $2^m$, i.e.,
\beq \underbar{v}_p(r) \leq  v(r') \leq \bar{v}_p(r) \quad \forall r' \geq r. \eeq




We note that any block $B$ not in $P_{\ell}(r)$ has the following upper bound on its votes for all of the future: 
\beq \bar{v}_{\emptyset}(r) := m - \underbar{v}_{P_{\ell}}(r). \eeq





The list confirmation policy is as follows. Let us assume without loss of generality that the list
$P_{\ell}(r) = \{B_1,...,B_p\}$ is  such that the lower-bound on the votes are ordered $\underbar{v}_1(r) \geq \underbar{v}_2(r) ...\geq \underbar{v}_p(r) $.

The list at level $\ell$ can be confirmed if the following condition holds at round $r$: 
\beq \underbar{v}_1(r)  \geq \bar{v}_{\emptyset}(r),  \label{eq:list_cond}\eeq
i.e., the dominant block is guaranteed to get more than any unseen block.  Under this condition, the confirmation policy is now defined as follows: 
\beqa p^* &=& \min_p \mathrm{s.t.} \bar{v}_p(r) < \underbar{v}_1(r). \\
\Pi_{\ell}(r) &=& \{B_1,...,B_{p^*}\}.
\eeqa

We note that the list $\Pi_{\ell}(r)$ has the property that the final leader block for level $\ell$ will be an element from this list, except with vanishingly small probability.

{\bf List decoding of ledger}

We can use  the list of proposer at each level to arrive at a list of ledgers, one of which is guaranteed to be a prefix of any future uniquely decoded ledger. 


Define the maximum level till which we have a valid list as follows: 
\beq \bar{\ell}(r) = \max {\ell} \textrm{ s.t. } \Pi_{\ell}(r) \textrm{ is well defined}. \eeq

We first define a ledger as a sequence of blocks one each from each consecutive level - here we do  not require the consecutive block to necessarily have a parent-child relationship. The ledger does not have internal validity because of the above property, i.e., it can have double-spends, however, since a ledger contains a total ordering of transactions, it can be sanitized to remove the double-spends (the second occurrence when a previous output is spent can be ignored).


We can define a list of ledgers as a Cartesian product as a list of blocks at each level, i.e., 
\beq \mathcal{L}(r) = \Pi_{1}(r) \times \Pi_{2}(r)  \times  \cdots \Pi_{\bar{\ell}}(r). \eeq

We note that we consider $\mathcal{L}(r)$ as a set of ledgers out of which the true ledger is an element. 
-------------

{\bf List confirmation latency}
We need to get an estimate on how much time is required to get a confirmation on a list at a given level $\ell$ from the time an initial proposal block is floated in public for that level. We now need to calculate when the list can be confirmed at this level, i.e., when condition \eqref{eq:list_cond} holds. Let there be $P_{\ell}(r)$ proposers at round $r$. Suppose $1-\theta$ fraction of the trees have already voted for this level $\ell$ and suppose other than $\mu m$ of these votes, the remaining are permanent. This implies that, 
\beqa  \underbar{v}_{P_{\ell}(r)}  \geq  \{1-\theta-\nu\}m  & \Rightarrow &
\bar{v}_{\emptyset}(r)  \leq  \{\theta + \mu \} m
\eeqa


Since the block with the maximum vote in $P_{\ell}(r)$ atleast should have $\frac{1}{P_{\ell}(r)}$ fraction of votes, we get
\beqa
\underbar{v}_{B_1}(r)  \geq   \{ \frac{1-\theta}{P_{\ell}(r)} - \nu \} m \eeqa

Now, by \eqref{eq:list_cond}. a list is formed when $\underbar{v}_{B_1}(r) \geq \bar{v}_{\emptyset}(r)$, i.e.,
\beqa
P_{\ell}(r)  \leq  \frac{1-\theta}{\theta+2 \nu}. \label{eq:P_bound}
\eeqa


According to Theorem~\ref{thm:latency_k_rounds}, we know that after $k$ rounds of the time when the first proposal block at level $\ell$ is introduced, $1-\theta$ fraction have already voted for level $\ell$ at depth $\alpha k$, where \beq 1-\theta = [1-2 e^{-\gamma k}](1-\delta).\eeq 

Theorem~\ref{thm:irreversibility} guarantees that atmost $\mu m$ of those votes are reversible, where 
\beq 1-\mu = (1-e^{-\gamma \alpha k}-e^{-\frac{\alpha k}{6}})(1-2\delta) \eeq

Given that $\delta = m^{-0.33}$, we can show that if $k< O(\log m)$, we can get
\beqa \theta \leq 3 e^{-\gamma k} \\
\mu \leq 4 e^{-\gamma' k}, \eeqa
where $\gamma' = \alpha \cdot \max \{\gamma , \frac{1}{6}\} $. Plugging it into \eqref{eq:P_bound}, we get, after $k$ rounds, the list is confirmed if,
\beq P_{\ell}(r) \leq a e^{-\gamma' k}, \eeq with $a = \frac{1}{11}$.












--------------
Throughput + latency section





Each point is a subsection
-> Has a main theorem
-> Sketch of key ideas
-> Proof using lemma-proposition

Description of list decoding

==> new_related.tex <==
\section{Related work}
\label{sec:related}

%%We discuss and compare our approach to several lines of work.


%%Prior approaches to increasing throughput and/or reducing latency can broadly be classified into three categories. 
%%The first increases throughput by increasing the mining rate (as well as forking); transactions are ordered either through %%novel fork choice rules or DAG structures. 
%%The second approach \emph{decouples} different processes within the consensus mechanism, such as proposal and validation. %%The third combines ideas from Byzantine fault tolerant (BFT) along with blockchains. 
%%As discussed in the introduction, the main design principle behind \scheme is a decoupling of the various functionalities of %%the blockchain; at the same time, it ultimately uses a DAG to order transactions.
%%In that sense, \scheme draws on conceptual insights from the first two strategies, while avoiding the associated challenges.
\noindent {\bf High-forking protocols}. 
% The first class of protocols aims to increase throughput by embracing forking, while ordering transactions either through new fork choice rules or DAG structures. 
Approaches to increase throughput and decrease latency by using more sophisticated fork choice and voting rules %to deal with the high-forking nature of the blocktree.
%Examples of such high-forking protocols include 
 \cite{ghost,inclusive,spectre,phantom,conflux}.
The earliest of these schemes  handles forking through a fork-choice rule that builds on the heaviest subtree \cite{ghost}. %The authors observed that in order to improve throughput, we must increase the block mining rate, $f$.  However, as $f$ grows, so too does the number of blocks mined in parallel, which are wasted under \bitcoin\!\!'s longest-chain fork choice rule, thereby reducing security.  \ghost\!\!'s heaviest-subtree rule allows the system to benefit from blocks that were mined in parallel by honest nodes since such blocks are counted in the main chain calculation. 
While  this scheme is shown to be secured against a $50\%$ purely private attack, it turns out to be  vulnerable to a public-private balancing attack \cite{ghost_attack}, essentially reducing the throughput performance back to that of Bitcoin's. %where the adversary can use minimal effort to split the  work of the honest nodes across two subtrees of equal weight, and then launch a private attack. It turns out that counting side-chain blocks in selecting the main chain allows the adversary to withhold earlier mined blocks and use them at later times to balance the growth of the two subtrees. We present an analysis of this attack in the Appendix and show that this attack restricts the mining rate $f$ of \ghost to be similar to that of \bitcoin\!\!, thus minimizing the advantage of \ghost\!\!.


Another popular idea is to add reference links between blocks in addition to traditional parent links, resulting in a DAG-structured blockchain. %Each block in a DAG can reference multiple previous blocks instead of a unique ancestor (as in \bitcoin\!\!). 
The  challenge is how to choose the reference links and how to obtain a total ordering of blocks from the observed DAG in a way that is secure. In a family of protocols, \inclusive\!\!, \spectre and \phantom, every block references all previous orphan blocks;  the reference links are interpreted in differing ways to give these different protocols.
%In \cite{inclusive}, the key observation is that the reference link structure provides enough information to emulate any main-chain protocol, while in addition providing the ability to pull in stale blocks into a valid ledger. However, the security guarantee remains the same as that of \bitcoin (namely, tending to zero as the mining rate grows), and it does not achieve optimal throughput.
\cite{inclusive} allows  emulation of any main-chain protocol but still does not achieve optimal throughput.  \spectre achieves low confirmation times (only for honest transactions) by interpreting the reference links as votes to compare between pairs of blocks \cite{spectre} -- on the flip side, it does not guarantee liveness for double-spends nor achieve consensus on total ordering. %Since complete ordering is important for core blockchain applications (e.g., cryptocurrencies), 
\phantom\, builds on \spectre to achieve consensus on a total ordering of transactions by having  participants topologically sort their local DAGs \cite{phantom}. The authors suggest that by combining \spectre and \phantom, one may be able to achieve low confirmation latency for honest transactions as well as eventual total ordering; apart from the conjectural nature,  some variants of \phantom\,  are vulnerable to liveness attacks \cite{conflux} and the combination still cannot confirm  non-contentious total ordering with fast latency. \conflux is another DAG-based protocol, based on a combination of \inclusive and \ghostnosp.   %whose goal is to increase throughput \cite{conflux}.  However, \conflux\!\!'s reference links are not used to determine where to mine blocks or how to confirm them; they are only used to include side-chain blocks into the main chain to improve throughput. The main chain itself is selected by the \ghost rule. 
Due to the vulnerability of \ghost to the balancing attack, the secured throughput of \conflux is limited to \bitcoin levels. 

Although \scheme uses a DAG to order transactions, it diverges from prior DAG schemes by separating block proposal from block ordering in the protocol. This helps because an adversarial party that misbehaves during block proposal does not affect the security of transaction ordering, and vice versa; \scheme provides a degree of {\em  algorithmic sandboxing}. 

% (See discussions in Section \ref{sec:thruput_disc}.)

% A conceptually different approach instead \emph{decouples} different processes within the consensus mechanism, such as proposal and validation. 
\noindent{\bf Decoupled consensus}.  
Our design approach  of {\em decoupling} the various functionalities of the blockchain, has appeared in differing guises in earlier works,  especially in decoupling the transactions. We review these works here.

%%The second class of consensus mechanisms algorithmically decouples different functionalities; some schemes that employ this %%approach include \bitcoinNG \cite{bitcoin-ng} and \fruitchains \cite{fruitchains}.

\bitcoinNG\!\!\cite{bitcoin-ng} elects a single leader to propose a predetermined number of transaction blocks, called an epoch. 
%At the end of this epoch, a new leader is elected. Thus, there is a decoupling of proposal blocks and transaction blocks, the goal being to increase the throughput.
\bitcoinNG is vulnerable to various security attacks, such as bribery or DDoS attacks, whereby an adversary can corrupt a block proposer after learning its identity. 
In contrast, \scheme does not reveal the identity of a block proposer \emph{a priori}.


% \red{
%In \bitcoinNGnosp, if the leader is malicious, it may try to double spend transaction blocks during its epoch. 
%Although this event is handled by the \bitcoinNG confirmation rule, which only confirms transactions once they are deep enough in the chain of keyblocks, the confirmation rule incurs a latency comparable to \bitcoinnosp's.
\byzcoinnosp~\cite{byzcoin} and its predecessor \disccoinnosp~\cite{disccoin} address the latency shortcoming of \bitcoinNG  by using BFT  protocols
% collective signing (CoSi) primitive \cite{cosi} 
in an architecture similar to \bitcoinNGnosp's.
% Like \bitcoinNGnosp, \byzcoin separates time into epochs, where 
% each epoch is associated with a new leader and validation committee; these are determined by the blockchain. 
% In a given epoch, the leader proposes frequent transaction blocks, which the committee commits (and signs). In parallel, a separate chain of infrequent, PoW keyblocks mark the end of each epoch, and the composition of the next committee. 
% Transaction blocks contain pointers to both the most recent transaction block and keyblock; all blocks are collectively signed \cite{cosi}, which prevents forking among transaction blocks. 
% Notably, \byzcoin transaction blocks are not mined but are put on the chain by the committee leader, and confirmed by a fixed committee.
% Hence, the leader and/or committee nodes remain subject to DDoS or bribery attacks. 
% }

The objective of \fruitchainsnosp \cite{fruitchains} is to provide fairness mitigating the selfish mining attacks of \bitcoinnosp  \cite{eyal2018majority,sapirshtein2016optimal,nayak2016stubborn}.
\fruitchains mechanically resembles Nakamoto consensus, except miners now mine separate mini-blocks, called fruits, for each transaction. Fairness is achieved because the fraction of fruits a miner can mine is proportional to its computational power. As in \bitcoinNGnosp, the fruits (transactions) are decoupled from the proposal blocks in the blocktree, but for a different reason: to improve fairness. 

\noindent{\bf Hybrid blockchain-BFT consensus}. 
Combining ideas from Byzantine fault tolerant (BFT) into blockchains is studied in \cite{hybrid,thunderella}.   \emph{Hybrid consensus} uses a combination of traditional mining under a longest-chain fork choice rule with Byzantine fault tolerance (BFT) consensus \cite{hybrid}, 
%The basic idea is that every $k$ blocks, a BFT protocol is run by an elected committee of nodes. 
designed to provide performance proportional to actual network performance. % rather than an \emph{a priori} bound on network delays.
%The authors show that no responsive protocol can be secure against more than $1/3$ adversarial power, and hybrid consensus achieves this bound. 
In this work, our focus is not on being responsive to network delay, but close to the propagation delay physical limit and small error probability.



%but assume a worst-case bound on network latency. 
%Under our (weaker) network model and system objectives, we provide security against up to $1/2$ adversarial power.  
%This BFT protocol confirms transactions in the preceding $k$ blocks. However, the protocol is only secure up to $33\%$ adversary power because it is based on BFT consensus. 
%%Although hybrid consensus has good throughput, it also exhibits a (comparatively) high confirmation latency due to the waiting period between BFT %%protocols. 
%% 
%% not sure this is true. I think the slow chain is run in parallel to the BFT.
A closely-related protocol called \thunderella includes a slow Nakamoto consensus blockchain, as well as a faster confirmation chain that is coordinated by a leader and verified by a BFT voting protocol \cite{thunderella}. 
 \thunderella achieves low latency under optimistic conditions, including having a honest leader and a $\beta < 0.25$, while having consistency under worst case condition ($\beta = 0.5$). In contrast, our protocol achieves low latency under all conditions, but for list-decoding  and  confirmation of honest transactions. 

% \red{Along similar lines, \byzcoin separates time into epochs, where 
% each epoch is associated with a new leader and validation committee; these are determined by the blockchain. 
% Each epoch runs a BFT-style algorithm where the leader proposes frequent transaction blocks, which are  signed by the committee. In parallel, a separate chain of infrequent, PoW keyblocks mark the end of each epoch, and the composition of the next committee. 
% Transaction blocks contain pointers to both the most recent transaction block and keyblock; all blocks are collectively signed \cite{cosi}, which prevents forking among transaction blocks. 
% Notably, \byzcoin transaction blocks are not mined but are put on the chain by the committee leader, and confirmed by a fixed committee.
% Hence, the leader and/or committee nodes remain subject to DDoS or bribery attacks.  }

%%\blue{VB: Byzcoin has a few security flaws and it is pointed out in Hybrid Consensus paper. Hybrid is Byzcoin done right.}
 
 
 %% We point out that in these protocols, the committees executing the consensus algorithms are elected based on leaders in the (slow) blockchain.  Furthermore, there is a hybrid mode - executing a consensus algorithm  In contrast in our protocol, the hybrid nature is manifest due to the separation of 
 
%Somewhat similar to these protocols, which have separate voting committees,  \scheme also has voting

\noindent {\bf Miscellaneous}. Our two-threshold protocol is  similar to the ones used in mining pools \cite{lewenberg2015bitcoin} - here   partial Proof-of-Work using a higher hash threshold is used by participants to prove that they have been working. % (since they may be unable to generate full proof-of-work messages at regular intervals). 
   
\scheme is reminiscent of  subchains \cite{subchains} or weak blocks \cite{weakblocks1,weakblocks2}: both  employ blocks with lower hash threshold (``weak blocks'') along with regular blocks. However unlike \schemenosp, these weak blocks have to form a chain structure and the corresponding  PoW rate of weak blocks is restricted to avoid  high forking. 
   
 We note that a version of transaction scheduling appears in Inclusive \cite{inclusive} for incentive compatibility. In order to maximize the reward gained, selfish users select a random subset of transactions to include in the ledger. In \scheme we show this is required to maximize transaction throughput, even with altruistic users.




    

==> random_walks_condensed.tex <==
% \section{Others}

% \begin{figure}
% \hspace{-.65in}
%   \includegraphics[width=1.2\linewidth]{figures/Reserve_blocks.pdf}
%   \caption{Number of reserved blocks by the adversary on level $\ell$ in round $\R_{\ell}.$ \label{fig:reserve}}
%  \end{figure}
 
% \subsection{Reserve proposer blocks by the adversary}\label{sec:reserve_blocks}
% Say the honest users mine the first proposer block at level $\ell$ in round $R_{\ell}$. Let $W_{\ell}^p(R_{\ell})$ denote that the number of hidden proposal blocks blocks on level $\ell$ by the adversary. In order to maximize  $W_{\ell}^p(R_{\ell})$, all these hidden proposer blocks should have a common honest parent proposer block at level (say) $\ell_{honest}$ linked via private proposal blocks as shown in the Figure \ref{fig:reserve}. The total number of reserve blocks is given by
% \begin{equation}
% W_{\ell}^p(R_{\ell}) = \max_{\ell_{honest}\leq \ell} Z^p[R_{\ell_{honest}}+1, R_{\ell}]-Y^p[R_{\ell_{honest}}+1, R_{\ell}]+1.
% \end{equation}

% The random variable $Y^p[R_{\ell_{honest}}, R_{\ell}]-Z^p[R_{\ell_{honest}}, R_{\ell}]$ is a random walk in the variable $\ell_{honest}$ with a net drift of $\frac{(1-2\beta)f_v}{2}$. The ratio of left drift to the right drift is $2\beta$ and from \cite{randomwalk}, we have 

% \begin{align*}
%     \mathbb{P}(W_{\ell}^p(R_{\ell}) > k) &=  \mathbb{P}\big(\max_{\ell_{honest}\leq \ell}Z^p[R_{\ell_{honest}}+1, R_{\ell}]-Y^p[R_{\ell_{honest}}+1, R_{\ell}]\geq k\big) \\
%      &=(2\beta)^{k}.
% \end{align*}
% Therefore $W_{\ell}^p(R_{\ell}) \sim \geom(1-2\beta)$. 



% \subsection{Random walk proofs}
% Consider the following event from Equation \eqref{eqn:single_chain_event}
% \begin{align*}
%     \tE_1\left[r - r', r\right] :=& \bigcap_{a,b\geq 0}\left\{ Y[r - r'-a, r+b] - Z[r - r'-a, r+b] > \frac{(1-2\beta)k}{8} \right\},\nonumber
% \end{align*}
% for $r'=\frac{k}{2\fv}$. The random variable $W[r-r',r] =  Y[r-r',r] - Z[r-r',r]$ is  a random walk with drift $\frac{(1-2\beta)f}{2}$. 
% % This random walk escapes to $\infty$ as $k\rightarrow \infty$ wp $1$.

% \begin{lemma} \label{lem:RW_1}
% If $W[r-r',r] > c_1k$, for $c_2<c_1$ we have
% \begin{align*}
%     \mathbb{P}\big(W[r-r', r+a] \geq c_2k \; \forall\; a >0) &= 1 - (2\beta)^{(c_1-c_2)k}\\
%     &= 1  - e^{\log (2\beta)(c_1-c_2)k}.
% \end{align*}
% \end{lemma}
% \begin{proof}
% Refer \cite{randomwalk}.
% \end{proof}


% If the random walk is to the right of $c_1k$ after $r'$ steps, 
% the above lemma calculates the probability of that the random walk remains to the right of $c_2k$ in all future rounds.

% \begin{lemma} \label{lem:RW_2}
% If $W[r-r',r] > c_1k$, for $c_2<c_1$, then we have
% \begin{align*}
%     \mathbb{P}\big(W[r-r'-b, r] \geq c_2k \; \forall\; b >0) &= 1 - (2\beta)^{(c_1-c_2)k}\\
%     &= 1  - e^{\log (2\beta)(c_1-c_2)k}.
% \end{align*}
% \end{lemma}
% \begin{proof}
% Refer \cite{randomwalk}.
% \end{proof}
% The above lemma is mathematically characterizing the same event as Lemma \ref{lem:RW_1}.

% \begin{lemma} \label{lemma:RW_3}
% If $W[r-r',r] > c_1k$,then for $c_3<c_1$, then we have
% \begin{align*}
%     \mathbb{P}\big(W[r-r'-b, r+a] \geq c_3k \; \forall\; a >0) &\geq 1 - 2(2\beta)^{(c_1-c_3)k/2}\\
%     &= 1  - 2e^{\log (2\beta)(c_1-c_3)k/2}\\
%     &\overset{(a)}{\geq} 1  - 2e^{-(1-2\beta)(c_1-c_3)k/2}.
% \end{align*}
% \end{lemma}
% \begin{proof}
% Using $c_2=(c_1-c_3)/2$ in the above two Lemmas \ref{lem:RW_1} and \ref{lem:RW_2}, we get the required result. The inequality $(a)$ uses $\log 2\beta < 2\beta -1$ for $\beta>0$.
% \end{proof}


==> related.tex <==
\section{Related Work}
\label{sec:related}

Existing consensus algorithms in the literature achieve different tradeoffs between throughput, latency, and security. 
In this section, we overview a representative suite of consensus algorithms, along with their respective performance guarantees. 
These protocols can roughly be categorized according to their \emph{fork choice rules}; that is, given a node's local view of the block tree, how does it choose where to append a new block? 
A common class of protocols uses a longest-chain fork choice rule, building atop Nakamoto consensus.
This fork choice rule finds the longest chain from the genesis block to a leaf of the block tree, and appends new blocks to this leaf. 
The second class of protocols uses a heaviest-subtree-based fork choice rule, building atop the insights of GHOST \cite{ghost}.
Under this fork-choice rule, proposers start at the genesis block, and at every fork in the block tree, they choose the fork with the most total nodes in the corresponding subtree.
These two approaches exhibit substantially different properties, both in terms of security and performance. 
We summarize all latency and throughput results in Table \ref{tab:related}, and include proofs for these results in Appendix \ref{app:related}.

\begin{table}[]
\begin{center}
\begin{tabular}{|l|c|c|c|}
\hline
\textbf{Algorithm}                              & \textbf{Throughput ($\lambda/C$)} & \textbf{Latency ($\tau/D$)} & \textbf{Security Threshold}\\ \hline
\begin{tabular}{@{}l@{}l@{}l@{}}Bitcoin \cite{bitcoin} \\ Fruitchains \cite{fruitchains} \\ 
Thunderella,  \\ (Pessimistic) \cite{thunderella} \end{tabular}         &    $\frac{1-2\beta}{1- \beta}$ &     $O\left(\log(\frac{1}{\epsilon})\frac{1}{(1-2\beta)^3} \right )$  & 1/2           \\ \hline
Bitcoin-NG \cite{bitcoin-ng}   &  1-\beta                   &     $O\left(\log(\frac{1}{\epsilon})\frac{1}{(1-2\beta)^3} \right )$             & 1/2 \\ \hline
\begin{tabular}{@{}l@{}}Thunderella \\ (optimistic) \cite{thunderella} 
\end{tabular}&                     &             &     \\ \hline
% Fruitchains \cite{fruitchains} &                     &                  \\ \hline
% Hybrid consensus \cite{hybrid} &                     &      $O\left ( \log(\frac{1}{\epsilon})\frac{(1+3\beta)}{(1-3\beta)^2}\right )$        & $<1/3$    \\ \hline
GHOST \cite{ghost}   & $\frac{1-2\beta}{1-\beta}$ &              &    \\ \hline
Conflux \cite{conflux}         &      $\frac{1-2\beta}{1-\beta}$               &   GHOST   &     GHOST       \\ \hline
Spectre \cite{spectre}         &                     &               &   \\ \hline
Phantom \cite{phantom}         &                     &               &   \\ \hline
\end{tabular}
\label{tab:related}
\caption{Throughput and latency metrics for existing consensus proposals, in terms of $\beta$, the fraction of adversarial users, and $\epsilon$, the probability of transaction confirmation reversal. The security threshold describes the fraction of malicious nodes that can be tolerated.}
\end{center}
\end{table}

\subsection{Longest-Chain Fork Choice Rule}
The first and most well-known protocol using a longest-chain fork choice rule is Nakamoto consensus, as seen in Bitcoin \cite{bitcoin}. 
This is the baseline against which we compare subsequent algorithms.
%A number of subsequent protocols improved upon Bitcoin's performance. 
An early example of a scheme building on Nakamoto consensus is Bitcoin-NG \cite{bitcoin-ng}, which elects a single leader to propose a predetermined number of sequential blocks, called an epoch. 
At the end of this epoch, a new leader is elected. 
As seen in Table \ref{tab:related}, Bitcoin-NG achieves higher throughput than Bitcoin, but this gain comes at the expense of worsened latency. 
The latency increase occurs because to confirm a transaction with probability $1-\epsilon$, a diverse set of proposers must confirm the block. 
Because new proposers are only chosen after each epoch in Bitcoin-NG (instead of every block as in Bitcoin), transaction confirmation latency is high. 

A later scheme called \emph{Fruitchains} also uses the longest-chain fork choice rule \cite{fruitchains}.
The purpose of Fruitchains is to provide better chain quality compared to Bitcoin; at a high level, chain quality refers to the fraction of blocks in the main chain belonging to the adversary.
In Bitcoin, adversaries can augment this fraction relative to their computational power by using strategic mining and block release policies, such as selfish mining \cite{eyal2018majority}.
Fruitchains mechanically resembles Nakamoto consensus, except miners now mine separate mini-blocks, called fruits, for each transaction.
We find that Fruitchains has a similar latency and throughput to Bitcoin; notice that Fruitchains was never intended to improve scalability. 

A follow-up to Fruitchains called \emph{hybrid consensus} uses a combination of traditional mining under a longest-chain fork choice rule with Byzantine fault tolerant (BFT) consensus \cite{hybrid}. 
The basic idea is that every $k$ blocks, a BFT protocol is run by an elected committee of nodes. 
This BFT protocol confirms transactions in the preceding $k$ blocks. 
Although hybrid consensus has good throughput, it also exhibits a (comparatively) high confirmation latency due to the waiting period between BFT protocols. 
A closely-related protocol called \emph{Thunderella} includes a slow Nakamoto consensus blockchain, as well as a faster confirmation chain that is coordinated by a leader and verified by a BFT voting protocol \cite{thunderella}. 
Although Thunderella achieves high throughput and low latency under honest behavior, a malicious leader can revert the performance metrics to Bitcoin levels. 
% Since we cannot assume that leaders will always b


%\paragraph{Bitcoin (Nakamoto consensus).}
%
%\paragraph{Bitcoin-NG.}
%
%\paragraph{Fruitchains.}
%
%\paragraph{Hybrid Consensus.}

\subsection{Heaviest-Subtree Fork Choice Rule}
The idea of building on the heaviest subtree was first introduced  in the GHOST scheme \cite{ghost}.
This paper observes that in order to reduce latency, we must increase the block production rate, $f$. 
However, as $f$ grows, so too does the number of blocks mined in parallel, which are wasted under the longest-chain fork choice rule, thereby reducing throughput. 
The heaviest-subtree rule allows the system to benefit from blocks that were mined in parallel by honest nodes since such blocks are counted in the main chain calculation.
We find that GHOST exhibits better throughput and latency than Bitcoin; however, we have identified an attack on GHOST that enables an adversary to delay transaction confirmation indefinitely. 
To the best of our knowledge, this attack has not been discussed in the literature.

The attack proceeds as follows. 
Suppose an adversary has fraction $\beta<\frac{1}{2}$ of computational power. 
The adversary's goal is to prevent the system from coming to consensus on a particular transaction, $x$. 
To this end, it tries to maintain two parallel subtrees; one in which $x$ is valid, and one in which it is invalid. 
The adversary therefore splits its computational power evenly to mine on both subtrees simultaneously. 
It does not immediately release any of its mined blocks.
As soon as the honest nodes release blocks in one subtree, the adversary releases as many pre-mined blocks in the opposite subtree.
Since the honest nodes now observe two subtrees of equal weight, they (a) cannot confirm or deny the validity of $x$, and (b) split their computational power evenly (in expectation) over the two branches.
This attack is quite practical, since the adversary can simply monitor the state of the public blockchain to execute the attack effectively.
REVISE ATTACK BASED ON VIVEK'S WRITEUP
\cite{ghost_writeup}.

The above attack applies to other schemes built on top of GHOST; as such we consider such schemes insecure. 
Nonetheless, for the sake of completeness, we include the performance guarantees of these subsequent schemes, some of which are considered leading contenders in terms of scalability. 
Conflux is one such scheme \cite{conflux}.
Ultimately, GHOST chooses a single main chain from the blocktree, it uses concurrent blocks only to determine the main chain's identity. 
Conflux instead incorporates concurrent blocks into the transaction sequence. 

Phantom attempts to achieve consensus on a total ordering of transactions via having  participants topologically sort their local DAGs \cite{phantom}. The scheme promises high throughput and low latency for honest transactions. However, apart from the high computational complexity of the sorting algorithm as well as incomplete formal guarantees of the main claims, a recent work \cite{conflux} demonstrates a liveness attack on Phantom.


%\paragraph{GHOST.}
%
%\paragraph{Conflux.}
%
%\paragraph{Spectre.}
%
%\paragraph{Phantom.}

% \begin{itemize}
%     \item Bitcoin
%     \item Bitcoin-NG
%     \item GHOST, Spectre, Phantom, Conflux
%     \item Avalanche
%     \item Fruitchain
%     \item Thunderella
% \end{itemize}


==> related_SK.tex <==
\section{Related Work}
\label{sec:related}

% In this section, we discuss and compare our approach to several lines of work.


Prior approaches to increasing throughput and/or reducing latency can broadly be classified into two categories. 
The first increases throughput by increasing the block production rate (as well as forking); transactions are ordered either through novel fork choice rules or DAG structures. 
The second approach \emph{decouples} different processes within the consensus mechanism, such as proposal and validation. 
As discussed in the introduction, the main design principle behind \scheme is a decoupling of the various functionalities of the blockchain; at the same time, it ultimately uses a (structured) DAG to order transactions.
In that sense, \scheme draws on conceptual insights from both strategies, while avoiding the associated challenges.


\subsection{High-Forking Protocols}
% The first class of protocols aims to increase throughput by embracing forking, while ordering transactions either through new fork choice rules or DAG structures. 
Examples of high-forking protocols include  GHOST \cite{ghost}, Inclusive \cite{inclusive}, Spectre \cite{spectre}, Phantom \cite{phantom}, and Conflux \cite{conflux}.
The earliest of these schemes, GHOST, handles forking through a fork-choice rule that builds on the heaviest subtree \cite{ghost}. The authors observed that in order to improve throughput in Bitcoin, we must increase the block mining rate, $f$.  However, as $f$ grows, so too does the number of blocks mined in parallel,  
which are wasted under Bitcoin's longest-chain fork choice rule, thereby reducing security.  


GHOST's heaviest-subtree rule allows the system to benefit from blocks that were mined in parallel by honest nodes since such blocks are counted in the main chain calculation. While it was shown in \cite{ghost} that GHOST is secured against a $50\%$ purely private attack, it turns out that GHOST is vulnerable to a public-private balancing attack \cite{ghost_attack}, where the adversary can use minimal effort to split the  work of the honest nodes across two subtrees of equal weight, and then launch a private attack. It turns out that counting side-chain blocks in selecting the main chain allows the adversary to withhold earlier mined blocks and use them at later times to balance the growth of the two subtrees. We present an analysis of this attack in the Appendix and show that this attack restricts the mining rate $f$ of GHOST to be similar to that of Bitcoin, thus minimizing the advantage of GHOST.


To improve security at high mining rates, another important idea is to add reference links between blocks in addition to traditional parent links, resulting in a DAG-structured blockchain. Each block in a DAG can reference multiple previous blocks instead of a unique ancestor (as in Bitcoin). The pertinent challenge is how to construct and confirm blocks.  The Inclusive protocol \cite{inclusive} proposes to include blocks outside the main chain by creating links not only to a parent node but to all orphan nodes that it knows of. {\bf However, the security guarantee remains the same as that of Bitcoin (namely, tending to zero as block production rate grows), and it does not achieve optimal throughput.} Spectre is a related scheme that achieves low confirmation times at the expense of not ordering transactions completely \cite{spectre}. Since complete ordering is important for core blockchain applications (e.g., cryptocurrencies), a later work, Phantom, builds on Spectre to achieve consensus on a total ordering of transactions by having  participants topologically sort their local DAGs \cite{phantom}. The authors suggest that by combining Spectre and Phantom, one may be able to achieve low confirmation latency with a total ordering of transactions. However, apart from the high computational complexity of Phantom's sorting algorithm as well as incomplete formal guarantees of the main claims, a recent work \cite{conflux} demonstrates a liveness attack on Phantom.
Although \scheme uses a DAG to order transactions, it diverges from prior DAG schemes by separating block proposal from block ordering in the protocol. This helps because an adversarial party that misbehaves during block proposal does not affect the security of transaction ordering, and vice versa; it provides a degree of algorithmic sandboxing. 

Conflux is another DAG-based protocol whose goal is to increase throughput \cite{conflux}.  However, Conflux's reference links are not used to determine where to mine blocks or how to confirm them; they are only used to include side-chain blocks into the main chain to improve throughput. The main chain itself is selected by the GHOST rule. Due to the vulnerability of GHOST to the balancing attack, the secured throughput of Conflux is limited to Bitcoin levels. 

\subsection{Decoupled Consensus}
% A conceptually different approach instead \emph{decouples} different processes within the consensus mechanism, such as proposal and validation. 
The second class of consensus mechanisms algorithmically decouples different functionalities; some schemes that employ this approach include Bitcoin-NG \cite{bitcoin-ng}, Fruitchains \cite{fruitchains}, Hybrid consensus \cite{hybrid}, and Thunderella \cite{thunderella}. 
% As discussed in the introduction, the main design principle behind \scheme is a {\em decoupling} of the various functionalities of the blockchain.
The decoupling in Bitcoin-NG and Fruitchains is less explicit than later algorithms like Hybrid consensus and Thunderella. 


Bitcoin-NG \cite{bitcoin-ng} elects a single leader to propose a predetermined number of transaction blocks, called an epoch. 
At the end of this epoch, a new leader is elected. Thus, there is a decoupling of proposal blocks and transaction blocks, the goal being to increase the throughput. However, since the transaction blocks are not mined but are put on the chain by the leader and after the leader is elected, this protocol is subject to a bribery attack on the leaders, whereby an adversary can corrupt a block proposer after learning its identity. 
In contrast, \scheme does not reveal the identity of a block proposer \emph{a priori}.

The objective of Fruitchains \cite{fruitchains} is to provide better chain quality compared to bitcoin; at a high level, chain quality refers to the fraction of blocks in the main chain belonging to the adversary.
In Bitcoin, adversaries can augment this fraction relative to their computational power by using strategic mining and block release policies, such as selfish mining \cite{eyal2018majority}.
Fruitchains mechanically resembles Nakamoto consensus, except miners now mine separate mini-blocks, called fruits, for each transaction. Fairness is achieved because the fraction of fruits a miner can mine is proportional to its computational power. As in Bitcoin-NG, the fruits (transactions) are decoupled from the proposal blocks in the blocktree. 

% \subsection{Hybrid consensus and Thunderella}

\emph{Hybrid consensus} uses a combination of traditional mining under a longest-chain fork choice rule with Byzantine fault tolerant (BFT) consensus \cite{hybrid}. 
The basic idea is that every $k$ blocks, a BFT protocol is run by an elected committee of nodes. 
Hybrid consensus is designed to provide \emph{responsiveness}, which describes systems whose performance depends on the actual network performance rather than an \emph{a priori} bound on network delays.
The authors show that no responsive protocol can be secure against more than $1/3$ adversarial power, and hybrid consensus achieves this bound. 
We do not focus on responsiveness in this work, but assume a worst-case bound on network latency. 
Under our (weaker) network model and system objecetives, we provide security against up to $1/2$ adversarial power.  
%This BFT protocol confirms transactions in the preceding $k$ blocks. However, the protocol is only secure up to $33\%$ adversary power because it is based on BFT consensus. 
%%Although hybrid consensus has good throughput, it also exhibits a (comparatively) high confirmation latency due to the waiting period between BFT %%protocols. 
%% 
%% not sure this is true. I think the slow chain is run in parallel to the BFT.
A closely-related protocol called \emph{Thunderella} includes a slow Nakamoto consensus blockchain, as well as a faster confirmation chain that is coordinated by a leader and verified by a BFT voting protocol \cite{thunderella}. 
Although Thunderella achieves high throughput and low latency under honest behavior, a malicious leader can revert the performance metrics to Bitcoin levels. 






    

==> terminology.tex <==
 Terminologies:

Proposer block at \textit{level} $\ell$. Leader block at level $\ell$ is the proposer block with most number of votes.

Voter blocks. \textit{Depth} of a voter block is the length of chain under it. The voter blocks are on $m$ voter blocktrees.

Tx blocks. Fruits.

bitcoin, use \bitcoin

Proof-of-Work (PoW)  (caps on P and W, no caps on o)

hashing power (instead of compute power)
    
    
X,Y, Z should be terms from bitcoin backbone paper. 


==> things_to_do.tex <==

1. Parameter choice
-> 

==> throughput.tex <==
\section{Approaching physical limits: throughput}
\label{sec:throughput}

%- introduce high throughput scheme (just transaction blocks outside the block tree, no voter chains

%- say something about security (Bitcoin security)

%- combine with smart scheduling to get optimal throughput

%- analysis of throughput-beta tradeoffs of Bitcoin and GHOST and compare with Pheonix

%- discuss tradeoff between throughput and latency of getting a transaction on the tree, and observe that the latency is proportional to speed of light delay independent of eps. (similar analysis as in the 82318.tex writeup)

%- This leads naturally to discuss the other part of the latency: the confirmation latency
%\input{/usr/sww/share/lib/texmf/tex/generic/dvips/epsf}





% \subsection{Bitcoin and GHOST throughput}

% In Bitcoin, in order to improve the throughput, we can increase one of two parameters: the POW rate $f$ or block-size $B$. By increasing the parameter $f$, the maximum adversarial fraction $\beta$ takes a hit.
% Upon increasing the block-size $B$, the propagation delay $\Delta$ also increases, which increases forking in the chain. \color{red}{Include calculation of bitcoin tx throughput.} Thus for bitcoin, there is a tradeoff between a given security guarantee $\beta$ and the maximum throughput efficiency $\bar{\lambda}:=\frac{\lambda}{C}$ that can be achieved. In particular, for bitcoin, it can be observed that that $\bar{\lambda}$ goes to zero as $\beta$ approaches $0.5$ (thus bitcoin supports vanishing throughput as the adversary fraction approaches $0.5$).

In this section, we study the optimal throughput $\lambda$ achievable under worst-case adversarial behavior for a given adversarial power $\beta$. 
% We give an answer to this question in this section. 
The main results are summarized in Figure \ref{fig:throughput_comparision}, which show plots of $\bar{\lambda} := \lambda/C$ versus $\beta$ for various protocols. The metric $\bar{\lambda}$ is the throughput as a fraction of the network capacity and is a measure of the efficiency of a protocol.
The plot shows upper bounds on the efficiency of two baseline blockchain protocols, \bitcoin and \ghost (a version of GHOST is used in Ethereum).
Note that the throughput efficiency of both protocols vanishes as $\beta$ approaches $0.5$. In contrast, we design a protocol, \schemelitenosp, which attains a throughput efficiency of $1-\beta$. This efficiency does not vanish as $\beta$ approaches $0.5$ and is in fact the best possible if only honest nodes are working. We will see that the difference between \schemelite and the two baseline protocols is that while the throughput of the two baseline protocols are {\em security-limited} for large $\beta$, the throughput of \schemelite is only limited by the physical network capacity for {\em all} $\beta < 0.5$.

\begin{figure}
\begin{centering}
% \includegraphics[width=3.5in]{figures/baselines.pdf}
\includegraphics[width=0.8\linewidth]{figures/Thruput_vs_beta_comparision.pdf}
\caption{Throughput efficiency versus $\beta$ tradeoff of baseline protocols and \schemelite\!\!. The tradeoffs for the baseline protocols are upper bounds, while that for \schemelite is exact.}
\label{fig:throughput_comparision}
\end{centering}
\end{figure}

\subsection{Baselines: \bitcoin and \ghost}
\label{sec:baselines}

We derive  upper bounds on the achievable throughput under worst-case adversarial behavior of two key baselines: \bitcoin and \ghost\!\!. Throughput can be altered by tuning two parameters: the mining rate $f$ and block size $B$.  We are interested in the maximum achievable throughput efficiency ($\bar{\lambda}:=\frac{\lambda}{C}$), optimized over $B$ and $f$. 
To simplify notation, we suppress the dependence of $\bar{\lambda}$ on $\beta$.



\subsubsection{\bitcoin\!\!}

The security and consensus properties of \bitcoin have been studied by Nakamoto \cite{bitcoin}, and formally by \cite{backbone} in the synchronous model, followed by the analysis of \cite{pss16} in the asynchronous model.
These works and others (e.g., \cite{ghost,bloxroute})
show that choice of $f$ and $B$ in Nakamoto consensus has tradeoffs. 
As the mining rate $f$ grows, forking increases and  the maximum tolerable adversarial fraction $\beta$ shrinks, 
Similarly, as the block size $B$ grows, the network delay $\Delta$ also grows, which causes forking.

An upper bound on the worst case throughput (worst case over all adversary actions) is  the rate at which the longest chain grows when no adversary nodes mine. The longest chain grows by one block in a round exactly when at least one honest block is mined. Hence the rate of growth is simply $\Pr(H(r) >0)$, i.e.  
\begin{equation}
1 - e^{-(1-\beta) f \Delta} \;\; \mbox{blocks per round},
\label{eq:btc_chain_growth}
\end{equation}
Notice that \eqref{eq:btc_chain_growth} is monotonically increasing in $f$; hence to maximize throughput, we should choose as high a mining rate as possible. 

However, we are simultaneously constrained by security.
For \bitcoin\!\!'s security, \cite{backbone} shows  that the main chain must grow faster in expectation than any adversarial chain, which can grow at rates up to $\beta f \Delta$ in expectation.
Hence we have the following (necessary) condition for security:
\begin{equation}
1 - e^{-(1-\beta) f \Delta} > \beta f \Delta. 
\label{eq:bitcoin_condition}
\end{equation}
Equation \eqref{eq:bitcoin_condition} gives the following upper bound on $f\Delta$, the mining rate per round:
$$
f\Delta <  \bar{f}_{\text{BTC}}(\beta), 
$$
where $\bar{f}_{\text{BTC}}(\beta)$ is the unique solution to the equation:
\beq
\label{eq:fp}
1 - e^{-(1-\beta) \bar{f}} = \beta \bar{f}.
\eeq
This yields an upper bound on the throughput, in transactions per second, achieved by \bitcoin as:
\begin{eqnarray}
\lambda_{\text{BTC}} & \le & [1 - e^{-(1-\beta) \bar{f}_{\text{BTC}}(\beta)}] B/\Delta \nonumber \\
& = & \beta \bar{f}_{\text{BTC}}(\beta) B/\Delta,
\label{eq:bc_ub}
\end{eqnarray}
where the last equality follows from \eqref{eq:fp}. Substituting in $\Delta = B/C + D$ and optimizing for $B$, we get the following upper bound on the maximum efficiency of \bitcoin:
$$
\bar \lambda_{\text{BTC}} \leq \beta \bar{f}_{\text{BTC}}(\beta), 
$$
achieved when $B \gg CD$ and $\Delta \gg D$.

Another upper bound on the throughput is obtained by setting $f$ at the capacity limit: $f = C/B$ 
(cf. \eqref{eq:stability}). Substituting into \eqref{eq:btc_chain_growth} and optimizing over $B$, this yields 
$$
\label{eq:ub2}
\bar \lambda_{\text{BTC}} \leq 1 - e^{\beta - 1}, 
$$
achieved when $f\Delta = 1$,  $B \gg CD$ and $\Delta \gg D$.

Combining the above two bounds, we get:
$$
\bar \lambda_{\text{BTC}} \leq \min \left \{ \beta \bar{f}_{\text{BTC}}(\beta),  1 - e^{\beta -1} \right \}
$$
This is plotted in Figure \ref{fig:throughput_comparision}. Note that for large values of $\beta$, the first upper bound is tighter; this is a {\em security-limited} regime, in which the throughput efficiency goes to zero as $\beta \to 0.5$. This is a manifestation of the (well-known) fact that to get a high degree of security, i.e. to tolerate $\beta$ close to $0.5$, the mining rate of \bitcoin must be small, resulting in a low throughput. \bitcoin currently operates in this regime, with the mining rate one block per $10$ minutes; assuming a network delay of $1$ minute, this corresponds to a tolerable $\beta$ value of $0.49$ in our model.

For smaller $\beta$, the second upper bound is tighter, i.e. this is the {\em communication-limited} regime. The crossover point is the value of $\beta$ such that 
$$ 1 - e^{\beta - 1} = \beta,$$
i.e.,  $ \beta \approx 0.43$.


\subsubsection{\ghost\!\!}

The \ghost \cite{ghost}  protocol uses a different fork choice rule, which uses the heaviest-weight subtree (where weight is defined as the number of blocks in the subtree), to select the main chain. 
To analyze the throughput of \ghost\!\!, we first observe that when there are no adversarial nodes working, the growth rate of the main chain of \ghost is upper bounded by the growth rate of the main chain under the longest chain rule. Hence, the worst-case throughput of \ghost\!\!, worst-case over all adversary actions, is bounded by that of \bitcoin\!\!, i.e.
\beq \label{eq:ghost_chain_growth}
1 - e^{-(1-\beta) f \Delta} \quad \mbox{blocks per round},
\eeq
(cf. \eqref{eq:btc_chain_growth}). Notice that once again, this bound is monotonically increasing in $f$ and we would like to set $f$ largest possible subject to security and network stability constraints. The latter constraint gives the same upper bound as \eqref{eq:ub2} for \bitcoinnosp:
\beq
\label{eq:ub2}
\bar \lambda_{\ghost} \leq 1 - e^{\beta - 1}. 
\eeq

We now consider the security constraint on $f$. Whereas our security condition for \bitcoin throughput was determined by a Nakamoto private attack (in which the adversary builds a longer chain than the honest party), a more severe attack for \ghost is a balancing attack, analyzed in Appendix A.  As shown in that analysis, the balancing attack implies that a necessary condition on $f$ for robustness against an adversary with power $\beta$ is given by:
\beq
\label{eq:bal}
\mathbb{E}[|H_1[r] - H_2[r]|] > \beta f \Delta,
\eeq
where $H_1[r], H_2[r]$ are two independent Poisson random variables each with mean $(1-\beta)f\Delta/2$.
Repeating the same analysis as we did for \bitcoin\!\!, we get the following upper bound on the maximum efficiency of \ghost\!\!:
\beq
\bar \lambda_{\ghost} \leq \beta \bar{f}_{\ghost}(\beta),
\eeq
where $\bar{f}_{\ghost}(\beta)$ is the value of $f\Delta$ such that \eqref{eq:bal} is satisfied with equality instead of inequality. 

Combining this expression with the network stability upper bound, we get:
\beq
\bar \lambda_{\ghost} \leq \min \left \{ \beta \bar{f}_{\ghost}(\beta),  1 - e^{\beta - 1} \right \}. 
\eeq
The throughput is plotted in Figure \ref{fig:throughput_comparision}. As in  \bitcoin\!\!, there are two regimes, communication-limited for $\beta$ small, and security-limited for $\beta$ large. Interestingly, the throughput of \ghost goes to zero as $\beta$ approaches  $0.5$, just like \bitcoin\!\!. So although \ghost was invented to improve the throughput-security tradeoff of \bitcoin\!\!, the mining rate $f$ still needs to vanish as $\beta$ gets close to $0.5$. The reason is that although \ghost is indeed secure against Nakamoto private attacks for any mining rate $f$ \cite{ghost}, it is not secure against balancing attacks for $f$ above a threshold as a function of $\beta$. When $\beta$ is close to $0.5$, this threshold goes to zero.


%%\subsection{Baseline (new)}

\subsection{\schemelitenosp: throughput-optimal protocol}

We propose a protocol, \schemelitenosp, that achieves optimal throughput efficiency $\bar \lambda = 1 -\beta$, which does not vanish as $\beta$ approaches $0.5$. We will build on \schemelite in Section \ref{sec:latency} to obtain our full protocol \scheme\!\!.

Forking is the root cause of \bitcoin\!'s and \ghost\!\!'s inability to achieve optimal throughput. In designing \scheme1.0, our key insight is that we can create a secure blockchain by running \bitcoin at low mining rate with little forking, but incorporate additional transaction blocks, created via sortition,  through reference links from the \bitcoin tree   (Figure \ref{fig:scheme_lite}). This allows us to decouple the throughput from the mining rate $f$, and can increase the former without increasing the latter. In the context of the overall deconstruction approach (Figure \ref{fig:parallelize}), this decoupling is achieved by decoupling the transaction blocks from the core blockchain. Let us call the blocks in the core \bitcoin blockchain {\em core blocks}. Later, when we discuss latency, we will further split the functionalities of the core blocks into proposer and voter blocks to build a more complex consensus protocol, but for now we will just run \bitcoin as the basic consensus mechanism.

\begin{figure}
   \centering
   \includegraphics[width=.8\linewidth]{figures/Prism_lite.pdf}
   \caption{\scheme1.0. Decoupling the transaction blocks from the core blocks in the \bitcoin blockchain.
   \label{fig:scheme_lite}}
 \end{figure}
 
We now describe the structure of \scheme1.0.

\begin{enumerate}
    \item There are two hash-threshold parameters $\alpha_c$ and $\alpha_t$, such that $\alpha_{c} \leq \alpha_t$. A node mines blocks using a nonce. If the hash is less than the stringent threshold $\alpha_c$, the block is a core block. If the hash is less than the relaxed threshold $\alpha_t$ but greater than $\alpha_c$, the block is transaction block. This is a sortition of blocks into two types of blocks, and the adversary does not know which type of block it is mining until after the block has been mined.
    \item The core blocks are used to determine the structure of the main chain. Each core block will reference several transaction blocks, that are then assumed to be incorporated into the ledger. 
    \item A block header consists of the following data items.
    \begin{enumerate}
        \item The hash pointer to the current core block on which it is mining. 
        \item Hash of  all the transaction blocks that the miner knows of and that have not been referenced in the current main chain. 
        \item Hash of all transactions to be included.
        \item Nonce.
    \end{enumerate}
\end{enumerate}

If the block is a transaction block, then the miner broadcasts the transactions along with the block header. 
% the hash-pointers to the current core block as well as the hash-pointers to transaction blocks are not used. 
If the block is a core block, then the miner broadcasts the list of transaction blocks.
% the list of transactions is not utilized.
We note that the structure of the blocktree shown in Figure~\ref{fig:scheme_lite} 
% allows us to only package the information necessary for each type of block. 
%%\red{Then what exactly is included in the hash puzzle? Just txs? Still there, but not used} 
The ordered list of transaction blocks is produced by ordering the transaction blocks in the order in which they are referenced by the core blocks in the main chain. For example, if the core blocks are $c_1,..,c_k$, and $R(c_i)$ denotes the list of referenced transaction blocks by $c_i$, then the ordered list is given by $R(c_1),..,R(c_k)$. From the ordered list of blocks, we produce an ordered list of transactions. From this ordered list of transactions, the ledger is produced by sanitizing this list to ensure that no transaction appears twice, and for every double spend, only the first spend is kept in the sanitized ledger. 


Now that the key components of the protocol have been mentioned, we now explain how the protocol is run by various nodes. 

\begin{itemize}
    \item Each new transaction  is broadcast to all the nodes in the network. 
    \item Each node maintains a queue of outstanding transactions. The input to the queue is observed transactions. A transaction is cleared from the queue if the node knows of a transaction block containing the transaction. 
    %%\red{**should we call this a set, since queues are connoted with FIFO processing among programmers, but we can clear transactions from the queue in any order? And what if the transaction block ends up not being in the main chain down the line, and the new main chain doesn't contain that tx? I think the tx should get put back in the queue, right?**}
    %% all transaction blocks will be eventually referenced by a core block.
    \item %Each node maintains a blocktree of observed core blocks, as well as all the transaction blocks it has heard of. 
    Each node maintains a blocktree of observed core blocks and transaction blocks. 
%    , as well as all the transaction blocks it has heard of. 
    \item A node attempts to mine its new block(s) on top of the current longest chain of core blocks in its local blocktree.
    
    \begin{enumerate}
        \item The node includes in its block all transactions from its transaction queue that are valid with respect to the ledger formed from the current longest chain of the core blocktree.
        \item The node gives reference links to all transaction blocks not currently referenced by its core main chain. 
    \end{enumerate}
    \item A node that hears of a block determines its validity by checking the hash. Unlike in \bitcoinnosp, there is no transaction validity check for a block, since the ledger is sanitized later.  
\end{itemize}

%including transactions from the referred transaction blocks  in order in the main chain. 


%If a transaction block is referenced by more than one main chain core blocks, then it will be ordered by the earlier core block. If a transaction output is spent in multiple transactions, only the first transaction in the ledger is counted.




%%\red{How is transaction validity checked during chain construction? Since we ultimately use the main chain from the core blocktree to make the ledger, I assume block authors could check validity with respect to the previous core block and all core or tx blocks that come before it?} 
%%\red{How is the "first transaction in the ledger" determined if conflicting transactions are at the same height? By the local timestamp at which each node sees the transactions?}
%%Rewards are distributed to the transaction blocks (note: heavy-blocks also get a reward since they %%automatically satisfy the light-block hash constraint).

In the context of the round-by-round synchronous model, the $H[r]$ honest blocks mined in the $r$th round are now split into $H^c[r] \sim \pois ((1-\beta) f_c \Delta) $ honest core blocks and $H^t[r] \sim \pois ((1-\beta) f_t \Delta) $ honest transaction blocks, where $f_c + f_t = f$. Similarly, the $Z[r]$ adversarial blocks mined in the $r$th round are split into $Z^c[r] \sim \pois (\beta f_c \Delta) $ adversarial core blocks and $Z^t[r] \sim \pois (\beta f_t \Delta) $ adversarial transaction blocks.  
	The parameters $f_c$ and $f_t$ can be specified by choosing the appropriate value of the hash threshold $\alpha_c$.
\subsection{Analysis}

We now analyze the proposed protocol in our  network model. It is clear that the security of the protocol is the same as the security of the \bitcoin core blockchain. By setting $f_c$ to be appropriately small (depending on $\beta$), we know that we can keep the core blockchain secure. More specifically, \cite{backbone} gives one such sufficient condition, obtained by requiring that the rate of arrival of uniquely successful rounds exceeds the rate of work of the adversary:
\beq
\label{eq:uhonest}
f_c\Delta < \frac{1}{1-\beta} \ln \frac{1-\beta}{\beta}
\eeq
%%\red{should this be in terms of $f_c$? This equation doesn't seem to appear in the throughput analysis. Why is it needed here? It is used here.}
Under this condition, \cite{backbone} showed that the longest chain satisfies the common-prefix property as well as has positive chain quality. Similar to the argument in \conflux\!\! \cite{conflux}, the honest blocks in the longest chain can provide a total ordering of {\em all} the blocks, not just the core blocks. Hence, the throughput is given by the overall mining rate $f = f_c + f_t$. By choosing $f_t$ such that we are at the capacity limit, i.e.  $f = C/B $, we can get a total throughput of $(1-\beta)C/B$ blocks per second, or $(1-\beta)C$ transactions per second, assuming a worst case that only honest blocks carry transactions.

This seems to give us the optimal throughput efficiency $\bar \lambda = 1-\beta$. However, there is a catch: blocks that are mined in the same round may contain the same transactions, since transactions are broadcasted to the entire network. In the worst case, we have to assume that blocks mined at the same round contain an identical set of transactions. In this case, mining more than one block per round does not add to the (useful) throughput. Hence,  
the throughput, in terms of number of non-redundant  blocks, is simply:
$$ \Pr(H[r] > 0) = 1 - e^{-(1-\beta)f\Delta} \quad \mbox{blocks per second}.$$
Comparing to \eqref{eq:btc_chain_growth}, we see that this is exactly the longest chain growth rate of \bitcoin\!\!. Since \schemelite can operate at $f = C/B$, we are achieving exactly the communication-limited throughput of \bitcoin (c.f. \eqref{eq:ub2}), i.e.
$$ \bar \lambda = 1 - e^{\beta -1}, \qquad \beta \in [0,0.5).$$
The difference with the  throughput-security tradeoff of \bitcoin is that \schemelite is operating at the communication-limited regime for $\beta$ all the way up to $0.5$; there is no security-limited regime anymore. This is because we have decoupled transaction blocks from the core blockchain and the throughput is not security limited. In particular, the throughput does not go to zero as $\beta$ goes to $0.5$. But we are still not achieving the optimal throughput efficiency of $\bar \lambda^* = 1 -\beta$. 

\subsection{Transaction scheduling \label{sec:tx_sch}}

To achieve optimal throughput, one can minimize the transaction redundancy in the blocks by scheduling different transactions to different blocks.  Concretely, one can split the transactions randomly into $q$ 
queues, and each honest block is created from transactions drawn from one randomly chosen queue. 
Thinking of each transaction queue as a color, we now have transaction blocks of $q$ different colors.   
%\red{We discuss how to implement such a division securely  in in Section \ref{}; for now, assume that each transaction is irreversibly mapped to a randomly-chosen color, and miners can only create a block of a single color at a time. Other than the fact that miners can only construct blocks of a single color, \schemelite is the same as before: there is a single blockDAG, which is constructed as in Figure \ref{fig:scheme_1.0}. We also assume that at each block, miners choose a block color uniformly at random. (How is this achieved in a way that can't be gamed, and doesn't require the blocks to contain txs of all colors, and then the final color is selected after the nonce is discovered?)}

	We will only have honest blocks with redundant transactions if two or more blocks of the same color are mined in the same round.  The number of honest blocks of the same color mined at the same round is distributed as Poisson with mean $(1-\beta)f\Delta/q$, and so the throughput of non-redundant blocks of a given color is
 $$1 - e^{-(1-\beta)f\Delta/q} \;\; \mbox{blocks per round}.$$
The total throughput of non-redundant honest blocks of all colors is
\beq
\label{eq:prism_thruput}
q \left [1 - e^{-(1-\beta)f\Delta/q}\right] \; \;  \mbox{blocks per round}.
\eeq
For large $q$, this approaches 
$$ (1-\beta) f\Delta \;\;\mbox{blocks per round},$$ 
which equals 
$(1-\beta)C$ transactions per second when we set $f = C/B$. Thus, we achieve the optimal throughput efficiency 
$$\bar \lambda^* = 1 -\beta.$$ 
This performance is shown in the upper plot in Figure \ref{fig:throughput_comparision}.

Interestingly, this maximum throughput of \schemelite can be achieved whatever the choice of the block size $B$. In contrast, the block size $B$ has to be set large compared to the bandwidth-delay product $CD$ to optimize the throughput in both \bitcoin and \ghost\!\!. This extra degree of freedom in \schemelite has significant implications on the tradeoff between throughput and transaction latency, which we turn to next. 


\subsection{Throughput-Latency tradeoff}\label{sec:thr_lat_tradeoff}

So far we have focused on achieving the maximum  throughput of \schemelitenosp, without regard to latency.  But transaction latency is another important performance metric. The overall latency experienced by a transaction in \schemelite is the sum of two components: 
%%\red{this isn't a sum--do you mean there are two kinds of latency we can characterize?}
%% it is a sum: first processing, then confirmation.
\begin{enumerate}
    \item \textbf{Processing latency} $\tau_p$:  the latency from the time the transaction enters the transaction queue to the first time a block containing that transaction is mined.
    \item \textbf{Confirmation latency} $\tau$:  the latency from the time the transaction is first mined to the time it is confirmed.
\end{enumerate}
We will discuss in great depth the confirmation latency in Section \ref{sec:latency}, but for now let us focus on the processing latency $\tau_p$. It turns out that there is a tradeoff between the throughput $\lambda$ and the processing latency $\tau_p$.

We can calculate $\tau_p$  by considering the dynamics of an individual transaction queue. Let us make the simplifying assumption that transactions enter this queue at a deterministic rate. For a given total throughput $\lambda$ and $q$, the number of transaction queues, the arrival rate into this queue is $\lambda/q$ transactions per second. For stability, these transactions must also be cleared at a rate of $\lambda/q$. Thus it takes time $q B/\lambda$ seconds to clear a block of $B$ transactions from the queue and enters the blockchain. Hence,
\beq
\label{eq:prism_latency_p}
\tau_p = \frac{qB}{\lambda} \quad \mbox{seconds}.
\eeq
On the other hand, from \eqref{eq:prism_thruput}, we see that the throughput $\lambda$, at the capacity limit,  is given by
\beq
\lambda = q \left [1 - e^{-(1-\beta)C\Delta/(Bq)}\right] \frac{B}{\Delta} \quad \mbox{transactions per second}
\eeq

We see that increasing with the number of transaction queues $q$ increases the throughput but also increases the processing latency , as the effective arrival rate decreases. Hence tuning $q$ can effect a tradeoff between throughput and latency. To see the tradeoff explicitly, we can eliminate $q$ from \eqref{eq:prism_latency_p} and \eqref{eq:prism_thruput} and obtain:
\beq
\label{eq:tradeoff}
\bar{\lambda} = \frac{1-\beta}{\bar{\tau}_p \log \left ( \frac{1}{1-\frac{1}{\bar{\tau}_p}} \right)} \qquad \mbox{$1 < \bar{\tau}_p < \infty$},
\eeq
where  
$\bar{\tau}_p := \frac{\tau_p}{\Delta}. $

We see that as $\bar{\tau}_p$ goes to infinity, the throughput efficiency $\bar{\lambda}$ approaches $1-\beta$, the maximum throughput derived in previous section. This maximum throughput does not depend on the choice of the block size $B$, and this fact is consistent with our previous observation. However, for a given latency $\tau_p$, the throughput achieved depends on the network delay $\Delta$, which does depend on the block size $B$. By choosing the block size $B$ small such that $B \ll CD$, $\Delta$ achieves the minimum value of the propagation delay $D$, optimizing the tradeoff. Under this choice of the block size $B$, \eqref{eq:tradeoff} becomes a tradeoff between $\bar{\lambda}$, the throughput as a fraction of network capacity, and $\bar{\tau}_p$, the processing latency as a multiple of the propagation delay (Figure \ref{fig:tradeoff}). Thus \schemelite is achieving throughput and processing latency {\em simultaneously} near their physical limits. Note that \bitcoin and \ghost are not only sub-optimal in their maximum throughput, their throughput-latency tradeoff is also much worse. In particular, to achieve a non-zero throughput efficiency, the block size of these protocols is much larger than the bandwidth-delay product $CD$,  and as a consequence, the processing latency of these protocols needs to be much larger than the propagation delay. 

The remaining question is whether the {\em confirmation} latency can also be made close to the propagation delay. This is not the case in \schemelite since its confirmation latency is the same as that of \bitcoinnosp. This latency scales with $\log 1/\eps$, where $\eps$ is the confirmation error probability; this security parameter $\log 1/\eps$  can be many multiples of the network delay.  The question is whether we can improve upon \schemelite to make the confirmation latency of the same order as the processing latency. This will be addressed in Section \ref{sec:latency}.


\begin{figure}
\centering
\includegraphics[width=\linewidth]{figures/Thruput_vs_proceesing_latency.pdf}
\caption{Tradeoff between $\bar{\lambda}$ and $\bar{\tau}_p$ for different values of $\beta$. Throughput is normalized as a fraction of the network capacity, and the processing latency is normalized as a multiple of the speed-of-light propagation delay.}
\label{fig:tradeoff}
\end{figure}


 

\subsection{Discussions}
\label{sec:thruput_disc}

 We discuss the relationships of our protocol with several existing protocols.
 
\begin{enumerate}
    

    \item \conflux\!\!\cite{conflux} separates {\em links} into two types: main-chain links and reference links, but all the {\em blocks} go into the same blocktree. As a result, the \conflux\!\!'s security is limited by \ghostnosp, and because \conflux is not done in conjunction with transaction scheduling, its throughput-$\beta$ tradeoff is exactly the same as that of \ghost shown in Figure \ref{fig:throughput_comparision}. In contrast,  \schemelite not only separates links into two types but also separates {\em blocks} into two types: core blocks, which go into the core blockchain, and transaction blocks, which are referenced by the core blocks. This separation allows the protocol to have high security and high throughput simultaneously. 
    \item \schemelite can be viewed as similar to \bitcoinNGnosp~\cite{bitcoin-ng} but avoiding the risk of bribery attacks since the core block does not control which transactions to put into the ledger. Moreover, the core blocks incorporate transaction blocks from various nodes, thus increasing decentralization and fairness, unlike \bitcoinNG where the leaders are entitled to propose blocks till a new leader comes up.
%%    \item \red{Algorithmically, \schemelite is most similar to weak blocks and %%subchains \cite{weakblocks1,weakblocks2,subchains}. Our transaction blocks can be thought of as weak blocks; indeed, the process of mining weak blocks by imposing a looser hash threshold is very similar to that of mining transaction blocks. A key distinction is that subchains do not consider the scheduling of transactions, and therefore cannot achieve optimal throughput.}
    \item \fruitchains\!\!\cite{fruitchains} was designed as a mechanism to increase reward fairness and  \schemelite is designed for a totally different purpose of maximizing throughput, but the structure of \schemelite has similarity to \fruitchainsnosp. The transaction blocks are roughly analogous to fruits, though there are a few differences. 
    % The fruit-set is stored directly inside the block in \fruitchains  but we only store references (hash-pointers) to transaction blocks in the core blocks in order to optimize for throughput.
    The fruits hang-off an earlier block in \fruitchains for short-term reward equitability, but we do not need that for throughput optimality. The 2-for-1 mining protocol \cite{backbone,fruitchains} used in \fruitchains is somewhat different from our protocol. But more importantly, as we saw, transaction scheduling is crucial for achieving optimal throughput but is not present in \fruitchainsnosp.
    \item Our two-threshold protocol is also similar to the ones used in mining pools \cite{lewenberg2015bitcoin}. Indeed, in mining-pools, partial Proof-of-Work using a higher hash threshold is used by participants to prove that they have been working (since they may be unable to generate full proof-of-work messages at regular intervals). 
   
    \item Our protocol is reminiscent of an approach called subchains \cite{subchains} or weak blocks \cite{weakblocks1,weakblocks2}. Both methods employ blocks with lower hash threshold (``weak blocks'') along with regular blocks. However, unlike our protocol, these weak blocks have to form a chain structure. Thus, if the PoW rate of weak blocks is increased significantly, it will lead to high forking on the weak blocks, thus leading to lower  throughput. 
   
   \item  We note that a version of transaction scheduling appears in Inclusive \cite{inclusive} for incentive compatibility. In order to maximize the reward gained, selfish users select a random subset of transactions to include in the ledger. In our protocol, we show this is required to maximize transaction throughput, even with altruistic users.
    
    
%%    A third approach, which has been discussed extensively in the Bitcoin community, is known as \emph{weak blocks} \cite{weakblocks1,weakblocks2} or \emph{subchains} \cite{subchains}.
%%Subchains are a PoW mining strategy for reducing forking in which miners can mine either weak blocks, which have a looser hash threshold, or strong blocks, with a more stringent threshold.
%%A sequence of weak blocks is known as a subchain. 
%%Although both subchains and \scheme  use blocks of different hash difficulties, 
%%subchains add both weak and strong blocks to a \emph{single} main chain, using the %%longest chain fork choice rule.
%%In contrast, \scheme maintains separate blocktrees for weak and strong blocks, with a carefully-designed structure.
%%This subtle difference significantly alters the security, latency, and throughput guarantees of subchains compared to \schemenosp.
%%In particular, it prevents subchains from achieving low confirmation latency, because the act of voting on a transaction still only happens in a single, longest-chain blockchain. 
%%Although weak blocks themselves do not solve the latency and throughput problem, they do introduce an important notion: block size affects propagation delay, and modeling this physical network effect can lead to more nuanced algorithm design. Indeed, we use this insight in our own model. 
%%}
    
     
\end{enumerate}


==> thruput_old.tex <==
\section{Approaching physical limits: Throughput}
\label{sec:throughput}

%- introduce high throughput scheme (just transaction blocks outside the block tree, no voter chains

%- say something about security (Bitcoin security)

%- combine with smart scheduling to get optimal throughput

%- analysis of throughput-beta tradeoffs of Bitcoin and GHOST and compare with Pheonix

%- discuss tradeoff between throughput and latency of getting a transaction on the tree, and observe that the latency is proportional to speed of light delay independent of eps. (similar analysis as in the 82318.tex writeup)

%- This leads naturally to discuss the other part of the latency: the confirmation latency
%\input{/usr/sww/share/lib/texmf/tex/generic/dvips/epsf}





% \subsection{Bitcoin and GHOST throughput}

% In Bitcoin, in order to improve the throughput, we can increase one of two parameters: the POW rate $f$ or block-size $B$. By increasing the parameter $f$, the maximum adversarial fraction $\beta$ takes a hit.
% Upon increasing the block-size $B$, the propagation delay $\Delta$ also increases, which increases forking in the chain. \color{red}{Include calculation of bitcoin tx throughput.} Thus for bitcoin, there is a tradeoff between a given security guarantee $\beta$ and the maximum throughput efficiency $\bar{\lambda}:=\frac{\lambda}{C}$ that can be achieved. In particular, for bitcoin, it can be observed that that $\bar{\lambda}$ goes to zero as $\beta$ approaches $0.5$ (thus bitcoin supports vanishing throughput as the adversary fraction approaches $0.5$).

\subsection{Baselines}

We begin by deriving the throughput of two key baselines: Bitcoin (Nakamoto consensus) and GHOST. 
Although neither scheme achieves state-of-the-art throughput, later schemes have built on the intuitions presented in these papers. 
We are interested in the maximum throughput that is achievable in a secure system:

\begin{definition}[Security]
Consider a transaction $tx$, which enters the system at time $t_0$.
We say that a blockchain system is \emph{secure} if for any $\eps>0$ and any transaction $tx$, there exists a $\tau(\eps, \beta)<\infty$ such that at time $t_0 + \tau(\eps, \beta)$, a computationally-unbounded observer of the global blockchain can correctly predict whether $tx$ will be included in the limiting blockchain of every honest node (as $t\rightarrow \infty$) with probability at least $1-\eps$.
\end{definition}
Throughput can be altered by tuning two parameters: the PoW rate $f$ and block size $B$. 
We are interested in the maximum achievable throughput efficiency ($\bar{\lambda}:=\frac{\lambda}{C}$), optimized over $B$ and $f$. 
To simplify notation, we suppress the dependence of $\bar{\lambda}$ on $\beta$.
The optimal throughput efficiency of these baselines compared to \scheme is plotted in Figure \ref{fig:thruput_baselines}.

\begin{figure}
\begin{centering}
\includegraphics[width=3.5in]{figures/baselines.pdf}
\caption{Throughput of baseline schemes compared to \scheme\!\!.}
\end{centering}
\label{fig:thruput_baselines}
\end{figure}

\paragraph{Bitcoin (Nakamoto Consensus).}
The security and consensus properties of Nakamoto consensus have been closely studied by Garay \emph{et al.} \cite{garay2015bitcoin} in the synchronous model, followed by the analysis of Pass \emph{et al.} in the asynchronous model \cite{pss16}.
These works and others (e.g., \cite{ghost,bloxroute})
show that choice of $f$ and $B$ in Nakamoto consensus has tradeoffs. 
As the mining rate $f$ grows, the maximum tolerable adversarial fraction $\beta$ shrinks, and forking increases.
Similarly, as the block size $B$ grows, the propagation delay $\Delta$ also grows, which causes forking.
The following proposition upper bounds the maximum achievable throughput of Bitcoin (over all $f$ and $B$) as a function of $\beta$, the fraction of adversarial compute power. 
\begin{prop}
Bitcoin's maximum normalized throughput $\overline \lambda_{\emph{BTC}}$ satisfies:
$$
\overline \lambda_{\emph{BTC}} \leq 
\begin{cases}
 \frac{1-\beta}{2-\beta} & \text{if } \beta \in \left [0,\frac{3-\sqrt 5}{2} \right ] \\
 \frac{1-2\beta}{1-\beta} & \text{if } \beta \in \left (\frac{3-\sqrt 5}{2}, 0.5 \right ]  
\end{cases}
$$
\label{prop:bitcoin_thruput}
\end{prop}
\begin{proof}
The proof relies on a result from \cite{ghost}, which characterizes the \textbf{expected??} growth rate of the longest chain in Nakamoto consensus:
\begin{lemma}[Bitcoin chain growth \cite{ghost}]
The \textbf{expected??} growth rate of the longest chain under Nakamoto consensus is at least 
\begin{equation}
\frac{(1-\beta)f}{1+(1-\beta)f \Delta} \text{ blocks per second.}
\label{eq:btc_chain_growth}
\end{equation}
\textbf{This is a lower bound but we need an upper bound! :(}
\label{lem:chain_growth_bitcoin}
\end{lemma}
Notice that \eqref{eq:btc_chain_growth} is monotonically increasing in $f$; hence to maximize throughput, we should choose as high a block rate as possible. 
However, we are simultaneously constrained by security.
For Bitcoin's security, \cite{backbone} implies that the main chain must grow faster in expectation than any adversarial chain, which can grow at rates up to $\beta f$ blocks per second in expectation.
Hence we have the following (necessary) condition for security:
\begin{equation}
\frac{(1-\beta)f}{1+(1-\beta)f \Delta} > \beta f. 
\label{eq:bitcoin_condition}
\end{equation}
Equation \eqref{eq:bitcoin_condition} gives the following upper bound on $f$:
$$
f\Delta < \frac{(1-2\beta)}{\beta(1-2\beta)}. 
$$
Combining this bound with the network stability condition in \eqref{eq:stability} and converting \eqref{eq:btc_chain_growth} to units of transactions per second, we choose the optimal $f$ for Bitcoin as
$$
f^*_{\text{BTC}} = \min \left \{ \frac{(1-2\beta)}{\beta(1-2\beta)}, 1+\frac{C}{B}\cdot D \right \}.
$$
Now there are two possibilities:
\begin{enumerate}
\item If $\frac{1-2\beta}{\beta(1-\beta)}<1$, or equivalently $\beta > \frac{3-\sqrt 5}{2}$, then optimizing over $B$ yields
$$
\bar \lambda_{\text{BTC}} \leq \frac{1-2\beta}{1-\beta}.
$$
%
\item If $\beta \leq \frac{3-\sqrt 5}{2}$, then optimizing over $B$ yields
$$
\bar \lambda_{\text{BTC}} \leq \frac{1-\beta}{2-\beta}.
$$
\end{enumerate}
\end{proof}

%As $f$ increases, the maximum tolerable adversarial fraction $\beta$ takes a hit.
%Upon increasing the block size $B$, the propagation delay $\Delta$ also increases, which increases forking in the chain. \color{red}{Include calculation of bitcoin tx throughput.} 
Proposition \ref{prop:bitcoin_thruput} shows that for Bitcoin, there is a tradeoff between the security guarantee $\beta$ and the maximum throughput efficiency that can be achieved. 
In particular, $\lim_{\beta \to 0.5} \bar \lambda_{\text{BTC}}=0$, so  Bitcoin supports vanishing throughput as the adversarial fraction approaches $0.5$.
This was also previously observed in \cite{}.

\paragraph{GHOST.}
Let $\beta^*:= \sup \{\beta \,:\, \bar \lambda > 0\}$ denote the maximum fraction of adversarial compute power under which the system can securely support nonzero throughput.
We saw with Bitcoin that for a fixed $\beta$, optimal throughput depends closely (implicitly) on $\beta^*$; the same is true of GHOST. 
%GHOST is known to be vulnerable to a \emph{balancing attack} that limits its $\beta^*$. 
We show in Appendix \ref{} that a \emph{balancing attack} \cite{} limits GHOST's adversarial tolerance $\beta^*_{\text{GHOST}}$, which gives the following:
\begin{prop}
For $\beta \in [0,0.5]$, GHOST's maximum normalized throughput $\bar \lambda_{\emph{GHOST}}$ satisfies:
\begin{equation}
\bar \lambda_{\emph{GHOST}} \leq 
\begin{cases}
\frac{2\log \left(\frac{1-\beta}{\beta}\right)}{1+4\log \left(\frac{1-\beta}{\beta}\right)} & \text{if } \beta(e^{(1-\beta)/2}+1)>1 \\
\frac{1-\beta}{2-\beta} & \text{else} 
\end{cases}.
\label{eq:ghost_thruput}
\end{equation}
\label{prop:ghost_thruput}
\end{prop}

\begin{proof}
The proof follows a similar structure to that of Proposition \ref{prop:bitcoin_thruput}.
In particular, we rely on a result from \cite{ghost} that lower bounds the growth rate of the main chain. 
\textbf{Need an upper bound, not a lower bound!}

\begin{lemma}[(GHOST chain growth, \cite{ghost}]
The growth rate of GHOST's main chain is at least
\begin{equation}
    \frac{(1-\beta)f}{1+2(1-\beta)f \Delta} \text{ blocks per second.}
\label{eq:ghost_chain_growth}
\end{equation}
\label{lem:ghost_chain_growth}
\end{lemma}
% \begin{proof}
% %Lemma \ref{lem:ghost_bitcoin} can be shown through a simple coupling argument. 
% %Consider two worlds that contain duplicate networks of nodes, and let the network delays and leader elections (i.e. time of mining and identity of miner for each block) be coupled across worlds.
% %In one world, the longest-chain rule is used; in the other, the GHOST fork choice rule is used.
% %Then for each sample path, the length of the main chain in the GHOST world is upper bounded by the length of the main chain the longest-chain world, since the longest-chain proposer has access to all the same blocks as the GHOST proposer, and always increases the main chain . 
% \end{proof}
Notice that once again, this bound is monotonically increasing in $f$.
Whereas our security condition for Bitcoin throughput was determined by a Nakamoto-style attack (in which the adversary builds a longer chain than the honest party), our security condition for GHOST depends instead on a balancing attack, analyzed in Appendix \ref{}. 
As shown in that analysis, the balancing attack implies that 
$$
\beta^*_{\text{GHOST}}=(1-\beta^*_{\text{GHOST}})e^{-f\Delta (1-\beta^*_{\text{GHOST}})/2}.
$$
Combining this security condition with the stability condition \eqref{eq:stability}, we have
\begin{equation}
f^*_{\text{GHOST}}\Delta = \min \left \{\frac{2}{1-\beta}\log \left (\frac{1-\beta}{\beta} \right ), 1 + \frac{C}{B}\cdot D \right \}
\label{eq:ghost_fstar}
\end{equation}

\end{proof}
Notice that this expression is an upper bound. 
Throughput is limited by the balancing attack on GHOST; however, there may be other (more severe) attacks that could further limit throughput.
Again, we have two cases:
\begin{enumerate}
    \item If $\beta(1+e^{(1-\beta)/2})>1$ (this transition happens at $\beta \approx 0.43$), then the first term  of \eqref{eq:ghost_fstar} applies. Substituting this into \eqref{lem:ghost_chain_growth} and converting to units of transactions per second gives a throughput of
    $$
    \lambda^*_{\text{GHOST}}=\frac{2\log \left ( \frac{1-\beta}{\beta}\right )BC}{\left (1+4\log \left ( \frac{1-\beta}{\beta}\right ) \right )(B+CD)}.
    $$
    Optimizing this expression over $B$ (taking $B\to \infty$) gives
    $$
    \bar \lambda^*_{\text{GHOST}} = \frac{2\log \left ( \frac{1-\beta}{\beta}\right )}{\left (1+4\log \left ( \frac{1-\beta}{\beta}\right ) \right )}.
    $$
    %
    \item Otherwise, if If $\beta(1+e^{(1-\beta)/2})\leq 1$, the second term in the minimization applies. In this case, we get the same expression as the corresponding one for Bitcoin, i.e., 
    $$
    \bar \lambda^*_{\text{GHOST}} \leq \frac{1-\beta}{2-\beta}.
    $$
\end{enumerate}

%%\subsection{Baseline (new)}

\subsection{\scheme1.0: Throughput optimal scheme}

We propose a scheme, that we name \scheme1.0, that achieves high throughput and at the same time achieve security guarantee of any $\beta<0.5$. We will build on \scheme1.0 in later sections to obtain our full protocol \scheme\!\!.

In designing \scheme1.0, our key insight is that we can create a secure blockchain by running \bitcoin at low mining rate, but incorporate additional transaction blocks into the main chain through reference links from the \bitcoin tree.   (Figure \ref{fig:scheme_1.0}). In the context of the overall deconstruction approach (Figure \ref{fig:parallelize}), we are decoupling the transaction blocks from the core blockchain, whose blocks still have the coupled functionalities of proposing and voting\footnote{In reality, the core blocks still carry transactions, but since there will be many more transaction blocks than core blocks, the core blocks carry a negligible fraction of the total throughput}. Let us call the blocks in the core \bitcoin blockchain {\em core blocks}.

\begin{figure}
   \centering
   \includegraphics[width=0.3\linewidth]{Fig4.png}
   \caption{\scheme1.0. Decoupling the transaction blocks from the core blocks in the \bitcoin blockchain.}
   \label{fig:scheme_1.0}
 \end{figure}
 
We now describe the structure of \scheme1.0.

\begin{enumerate}
    \item There are two hash-threshold parameters $\alpha_c$ and $\alpha_t$, such that $\alpha_{c} \leq \alpha_t$. A node mines blocks using a nonce. If the hash is less than the stringent threshold $\alpha_c$, the block is a core block. If the hash is less than the relaxed threshold $\alpha_t$ but greater than $\alpha_c$, the block is transaction block. This is a sortition of blocks into two types of blocks, and the adversary does not know which type of block it is mining until after the fact.
    \item The core blocks are used to determine the structure of the main-chain. The transaction blocks Each core block will reference several transaction blocks, that are then assumed to be incorporated into the ledger. 
    \item A block comprises of the following data items.
    \begin{enumerate}
        \item Public-key for reward
        \item Transactions
        \item The hash pointer to the current core block on which it is mining. 
        \item Hash pointers (references) to sub-blocks that the miner knows of and that have not been referenced in the current main chain. 
        \item Nonce, which is mined by miners.
    \end{enumerate}
\end{enumerate}

If the block is a transaction block, then the hash-pointers to the current core block as well as the hash-pointers to the sub-blocks can be neglected.  Given these blocks, the ledger is produced by including transactions from the referred transaction blocks as well as the transactions in each core block in order in the main-chain. If a transaction output is spent in multiple transactions, only the first transaction in the ledger is counted. 
%%Rewards are distributed to the transaction blocks (note: heavy-blocks also get a reward since they %%automatically satisfy the light-block hash constraint).

In the context of the round-by-round synchronous model, the $X_i$ honest blocks mined in the $i$th round are now split into $X_i^c \sim \poiss ((1-\beta) f_c \Delta) $ honest core blocks and $X_i^t \sim \poiss ((1-\beta) f_t \Delta) $ honest transaction blocks, where $f_c + f_t = f$. Similarly, the $Z_i$ adversarial blocks mined in the $i$th round are split into $Z_i^c \sim \pois (\beta f_c \Delta) $ adversarial core blocks and $Z_i^t \sim \pois (\beta f_t \Delta) $ adversarial transaction blocks.  The parameters $f_c$ and $f_t$ can be specified by choosing the appropriate value of the hash threshold $\alpha_c$. 

\subsection{Analysis}

We now analyze the proposed protocol in the context of our simple network model. Suppose the POW rate is $f$ (blocks-per-second) for producing heavy blocks; then the POW rate is $mf$ for producing light blocks. It is clear that the security of the scheme is the same as the security of the main chain.


The maximum capacity constraint for our scheme translates to  $mfB = C$
and for a given $m$ and $B$ we set $f$ according to this equation. Since we are using a longest-chain protocol, due to the presence of forking, the growth rate of the main chain is,
$\frac{(1-\beta)f}{1 + (1-\beta)f\Delta} $ blocks per second.
 In order to guarantee security against $\beta$ fraction of adversaries this growth rate should be greater than $\beta f$, which is the adversarial growth rate. Hence, we need, for security, $
 \frac{(1-\beta)f}{\beta f}  > \frac{1}{1 + (1-\beta)f\Delta}
 $.
Indeed, it is known that Bitcoin is secure under a related constraint \cite{PSS16}:
\beqa \frac{1-\beta}{\beta} > \frac{1}{ 1- 2f\Delta}  \iff
\frac{1}{m} \left[1 + \frac{CD}{B} \right] < 0.5 \frac{1-2\beta}{1-\beta}, \eeqa
where we used $\Delta = \frac{B}{C}+D$. For any given $B$, $m$ can be chosen so that the above equation is satisfied. 

The transaction rate is now given by $mB$ times the growth rate of chain, which is  
\beqa \mathrm{Transaction Rate} & =&    \frac{m (1-\beta)fB}{1+(1-\beta)f\Delta} 
  =    (1-\beta)C \frac{\bar{m}}{\bar{m}+1}, \label{eq:tr_rate}
\eeqa
by choosing $m = \bar{m}(1-\beta)\left[ 1 + \frac{CD}{B} \right]$.

Some of the transactions are redundant in this list, and that leads to a loss in the effective transaction throughput. This is  because blocks proposed within $\Delta$ time of each other will contain overlapping transactions. There are $mf\Delta$ light-blocks proposed in $\Delta$ time. In order to minimize the overlap, we would like to keep $mf\Delta$ as close to $1$ as possible. 
$mf\Delta = mf \left[\frac{B}{C}+D \right]  = \left[1+ \frac{CD}{B} \right] $.
If we choose $B = \bar{k}CD$ for some constant $\bar{k}$, then the fraction of non-repeated transactions is $\frac{\bar{k}}{\bar{k}+1}$. 
Thus the transaction efficiency, which is transaction throughput normalized by capacity, is given by 
\beqa \bar{\lambda} =  \frac{\lambda}{C} & =&    (1-\beta) \frac{\bar{m}}{\bar{m}+1} \frac{\bar{k}}{\bar{k}+1}.
\eeqa



The latency for block-propagation is $\Delta  = \frac{B}{C}+D = D (1+k)$. The latency for a transaction getting to a block is then given by the waiting time for the next heavy block to be produced, which is 

\beq \tau = \frac{mB}{\lambda} \leq (\bar{m}+1) (\bar{k}+1) D \eeq

Note that for confirmation with a confirmation-probability $\eps$, we need to ensure that several heavy-blocks  are produced, which is a further component in the delay. Thus it is possible to achieve near optimal throughput $(1-\beta)$ with our scheme for arbitrary $\beta < 0.5$. This comes at a tradeoff with increasing latency. 

\subsubsection{Transaction Scheduling}
It is possible to improve the throughput-latency tradeoff by minimizing the overlap between transactions by using transaction scheduling. The basic insight is that since different miners are producing $m f \Delta$ blocks simultaneously, it is better to avoid overlap by choosing different transactions. We propose a transaction scheduling scheme, where each miner chooses each transaction in its transaction queue randomly with probability $\frac{1}{m}$. This leads to an expected overlap of $f \Delta B$ transactions in a total of $m f\Delta B$ transactions, thus leading to an efficiency of $\frac{m-1}{m}$. We get the transaction efficiency 
\beq \bar{\lambda} = \frac{\lambda}{C} = \frac{(m-1)(1-\beta)}{m+(1-\beta)\left[1+\frac{CD}{B}\right]} = (1-\beta)\frac{\bar{m}}{\bar{m}+1}, \eeq
where we have defined $\bar{m}$ based on $(m+1) = \bar{m}(1-\beta)\left[ 1+\frac{CD}{B} \right]$.

The delay now increases due to the waiting time of scheduling. In particular, if we assume that the transactions are entering at rate $\lambda$, then they are also clearing at rate $\lambda$ in steady state. However, each transaction gets picked to be in a block only with probability $\frac{1}{m}$, thus the overall latency is $\frac{mB}{\lambda}$. Thus the latency is 

\beq \tau = (\bar{m}+1) \left[ \frac{B}{CD}+1 \right] D \approx (\bar{m}+1) D, \eeq
where we have chosen $B$ much smaller than $CD$ to get the approximation. 







\subsection{Discussions}


\begin{enumerate}
    

    \item Unlike Conflux, which tries to separate links into two types: main-chain links and reference links, in \schemelite we separate {\bf blocks} into two types: core blocks, which go into the core blockchain and transaction blocks, which are referenced by the core blocks. 
    \item \schemelite is similar to Fruitchains \cite{fruitchains}: the transaction blocks are similar to fruits. Fruitchains was designed as a mechanism to increase reward fairness but \schemelite is designed to maximize throughput, and hence there a few differences. The fruit-set is stored directly inside the block in fruitchain but we only store references (hash-pointers) to transaction blocks in the core blocks in order to optimize for throughput. The fruits hang-off some earlier block in Fruitchains for short-term reward equitability, but we do not need that for throughput optimality. The 2-for-1 mining scheme \cite{backbone,fruitchains}used in fruit-chain is somewhat different from our scheme,
    \item \schemelite can be viewed as similar to Bitcoin-NG  but avoiding the risk of bribery attacks since the core block does not control which transactions to put into the ledger. Moreover, the core blocks incorporate transaction blocks from various nodes thus increasing decentralization and fairness, unlike Bitoin-NG where the leaders are entitled to propose blocks till a new leader comes up.
    \item Our two-threshold scheme is similar to the ones used in mining pools. Indeed, in mining-pools, partial Proof-of-Work using a higher hash threshold is used by participants to prove that they have been working (since they may be unable to generate full proof-of-work messages at regular intervals). 
     
\end{enumerate}


==> tx_structure_backup.tex <==

\begin{enumerate}
    \item {\em Links to proposer blocks}: If a block becomes a voter block, then it needs to vote on proposer blocks at various levels. Therefore the block contains votes of the form $(\ell, p_{{\ell}})$ for $\ell \in \{\ell_{\text{min}}, \ell_{\text{max}}\}$ where $p_{\ell}$ is a hash of a  proposer-block on level $\ell$. The honest strategy is to vote on the block on level $\ell$ that it heard about the earliest.  
    \begin{itemize}
        \item {\em Overloading}: If the block becomes a proposer-block, then the vote $p_{\ell_{\text{max}}}$ will certify that the block is at level $\ell_{\text{max}}+1$. 
    \end{itemize}
    
    \item {\em Parent block in each voter blocktree}: A block specifies  one parent in each voter blocktree, $B_i, i=1,2,...,m$. 
    Honest nodes choose $B_i$ as the leaf node in the longest chain of blocktree $i$. 
    If a block ultimately ends up in voter blocktree $i$, then it is attached to voter block $B_i$. 
    \begin{itemize}
        \item {\em Overloading}: If the block becomes a proposer-block,then  $B_1,..,B_m$ are treated as (implicit) reference links. 
    \end{itemize}
    
    
    \item {\em Other reference links}: A block also contains other reference links to blocks that it has seen but have not yet made it to the main chain. We term these blocks $R_1,...,R_j$, where $j$ is the number of reference links.
    \red{THis needs more detail. What other blocks? Are these on the proposer tree or voter trees? } 
\item {\em Transactions}: Each block contains transactions that have not yet been included in the main-chain (from the transaction queue). \red{(Do you mean have not yet been included in the transaction ledger? If not, which main chain are you referring to? proposer blocktree?)} The honest nodes utilize transaction scheduling  given in Section~\ref{sec:tx_sch} to choose a random subset of transactions.

\item {\em Nonce}: The nonce is a string discovered during PoW mining that seals the block; a valid nonce ensures that the hash value of the block (concatenated with the nonce) is less than a predetermined threshold. Our sortition mechanism uses the value of the hash to decide what type of block it becomes. In particular, we produce a  sortition as follows: 
  \begin{itemize}
      \item Hash $<\tau_p \Rightarrow$ Block is a proposer.
      \item $\tau_{v_{i-1}} < \text{Hash} < \tau_{v_{i}} \Rightarrow $ Block belongs to voter blocktree $i$ .
      \item The proposer PoW rate $f_p$ will be proportional to $\tau_p$, and if we want the voter PoW rate $f_v$ to be the same for all the blocks, this can be controlled using a single parameter $\tau_v$, and setting the parameters as follows,
      \begin{equation}\tau_{v_{i}} = i \tau_v + \tau_p, \quad i=1,2,..,m. \end{equation}
  \end{itemize}
    
\end{enumerate}

==> typicality.tex <==
\newpage
\section{Typical Execution}

The notion of typical execution plays an important role in the analysis in  the backbone protocol paper \cite{backbone}. We modify this notion for analyzing short latency confirmation.

The random variables in the problem are $Y_{rj}$ and $Z_{rj}$, where $r$ is the round and $j$ is the tree index. $r$ ranges from $1$ to $L$ and $j$ ranges from $1$ to $m$. Define typicality as follow: 

Let $S$ be a consecutive interval of rounds. Let $U^S_j = (Y_{rj}, Z_{rj})_{r \in S}$ be a 2 $|S|$ dimensional vector , a collection of all the randomness for tree $j$ over the interval $S$. Let $\hat{P}^S_m$  be the empirical distribution of the samples $U^S_1,.......U^S_m$ over the $m$ trees. Note that the empirical distribution removes the ordering information across the $m$ trees, which we don't care about since we are only interested in the fraction of trees in which good thing happen. Put it another way, the performance metrics we are interested in are label-invariant, i.e. we don't care about the tree that a vote comes from. So I believe the empirical distribution is a sufficient statistic for our problem. Note also that random variables like the fraction of trees that satisfies $Z_j(S) < Y_j(S)$ we were talking about earlier are functions of the empirical distribution $\hat{P}^S$.

Let $P^S$ be the (true) distribution of $U^S_1$. Note that $U^S_1, U^S_2, \ldots, U^S_m$ are i.i.d. random vectors. 

An execution is said to be typical on $S$ if $\hat{P}^S_m$ is close to $P^S$. 

An execution is said to be typical if it is typical on all $S$ of size $o(\log m )$ in the interval from $1$ to $L$. 

By a law of large number argument, we know that an execution is typical on $S$ with high probability for $m$ large and $|S| = o(\log m)$. If $L$ grows only polynomial of $m$ and since there are at most $L^2$ such $S$, by a union bound we also have typicality with high probability.

I believe this typicality is sufficient for our analysis of short latency confirmation, since we are only analysing the dynamics over intervals, and I am conjecturing that $o(\log m)$ lengths for these intervals are sufficient.



